FLEX: Feature Importance from Layered Counterfactual Explanations

Machine learning models achieve state-of-the-art performance across domains, yet their lack of interpretability limits safe deployment in high-stakes settings. Counterfactual explanations are widely used to provide actionable "what-if" recourse, but they typically remain instance-specific and do not quantify which features systematically drive outcome changes within coherent regions of the feature space or across an entire dataset. We introduce FLEX (Feature importance from Layered counterfactual EXplanations), a model- and domain-agnostic framework that converts sets of counterfactuals into feature change frequency scores at local, regional, and global levels. FLEX generalises local change-frequency measures by aggregating across instances and neighbourhoods, offering interpretable rankings that reflect how often each feature must change to flip predictions. The framework is compatible with different counterfactual generation methods, allowing users to emphasise characteristics such as sparsity, feasibility, or actionability, thereby tailoring the derived feature importances to practical constraints. We evaluate FLEX on two contrasting tabular tasks: traffic accident severity prediction and loan approval, and compare FLEX to SHAP- and LIME-derived feature importance values. Results show that (i) FLEX's global rankings correlate with SHAP while surfacing additional drivers, and (ii) regional analyses reveal context-specific factors that global summaries miss. FLEX thus bridges the gap between local recourse and global attribution, supporting transparent and intervention-oriented decision-making in risk-sensitive applications.

==> NLDL_2026/to_do.tex <==
\

1. Fix references

2. Think of potential advantages
    a) Simplicity
    b) Tying global and local with one approach
    c) Intuitive - humans understand counterfactuals, 
    d) Tailorable to different counterfactual properties eg actionable changes


3. Work to do
    a) [DONE] Decide on name: Multi-level Counterfactuals (CF) / Feature importance / Local / global
    b) Updating paper
        * Condense traffic stuff
        * Add second case study
        * Content on comparison with SHAP and possibly LIME
        * Update discussion


Global-Local explanation via counterfactuals: GLEC
FLEX – Feature importance from Layered (or Local/Global) EXplanations (suggests flexible/tailorable)
ReFLEX - Robust Feature importance & Local/global EXplanations (suggests flexible/tailorable)

==> SoGood_Workshop_Submission/sections/01_introduction.tex <==
\section{Introduction}
Machine learning models, particularly deep neural networks and ensemble methods, now regularly achieve state-of-the-art performance across diverse tasks. However, their internal decision processes remain opaque, earning them the designation of “black box” models. This opacity raises concerns around trust, accountability, and safety, especially in high-stakes domains including traffic safety \cite{guidotti2024counterfactual}.
Explainable AI (XAI) seeks to address these concerns by developing methods to interpret model behaviour. Among these, counterfactual explanations are especially intuitive and actionable.


A counterfactual explanation explores “what-if” scenarios by asking how targeted changes to input features would alter the model’s prediction \cite{wachter2017counterfactual}. Formally, given an instance $X$ with model output $a(X)$, a counterfactual $X'$ satisfies $a(X')\neq a(X)$, often whilst minimizing $||X'-X||$. This approach reveals the minimal adjustments needed to change the decision.

In traffic safety, understanding how to reduce accident severity is critical. Collisions are influenced by factors such as vehicle speed, weather, road design, and driver behavior. Prediction models alone do not identify effective interventions. Counterfactual analysis enables scenario-based reasoning—for example, “How could accident severity have been reduced?” or “What if the road were dry?” to observe the impact of individual features and guide targeted safety measures. Counterfactuals can provide explicit, actionable recommendations for transforming severe accident scenarios into non-severe ones.
Counterfactual explanations enhances model interpretability by producing feasible and cost-effective suggestions while minimizing changes to input features.

However, while counterfactuals can provide scenarios to change an outcome, there is usually no indication of feature importance. Additionally, the importance of a feature could vary depending on the region of the data space that a specific scenario occupies.
To address this, we present a framework for generating global and regional feature importances from counterfactual explanations. Globally, feature importance is assessed by how frequently a feature must be modified to change an accident severity prediction from “severe” to “non-severe.” Regionally, multiple counterfactuals are generated per instance and its neighborhood to identify region-specific contributing features to accident severity.
%This paper presents a framework for generating global and local counterfactual explanations for a random forest classifier trained on 12,316 traffic accident records from Addis Ababa, Ethiopia, collected between 2017 and 2020. Globally, feature importance is assessed by how frequently a feature must be changed to flip a severity prediction from “severe” to “non-severe.” Locally, multiple counterfactuals are generated per instance and its neighborhood to identify case-specific drivers of severity. The Pearson correlation coefficient quantifies the alignment between global and local importance; explanation sparsity and shifts in dominant feature categories are also analyzed. Results show that counterfactual explanations clarify model reasoning and offer actionable insights for reducing accident severity.


The main contributions of the paper are:
\begin{enumerate}
    \item Comparison of global and regional feature importance using feature change frequency of counterfactual explanations.
    \item Demonstrating our method on traffic accident records from the Addis Ababa dataset \cite{bedane2024road}.
    \item Offering actionable insights for reducing accident severity.
\end{enumerate}

 With further work and input from domain experts, these contributions could be applied to provide utility for policy makers aiming to introduce safety measures to reduce accident severity and save lives.

==> SoGood_Workshop_Submission/sections/conclusion.tex <==
\section{Conclusion and future work}
A global and regional counterfactual explanation framework was developed and applied to traffic accident data from Addis Ababa Sub-city police departments (2017–2020), revealing insights into feature importance for determining accident severity.

Global analysis identified $Driving\ Experience$, $Cause\ of\ Accident$, and $Types\ of\ Junction$ as the most frequently adjusted features needed to shift predictions from “severe” to “minor” accident severity, establishing a clear ranking of overall importance.
Analysis of regions, each composed of accidents with shared feature values, highlighted context-specific severity factors. These included features of particular importance in rainy weather conditions and issues linked to both experienced and inexperienced drivers, and identified feature values which may have reduced accident severity. Pearson correlation coefficient values between global and regional change frequencies ranged from 0.33 to 0.66, indicating that localised regional cases often deviate from wider trends.

These findings demonstrate that counterfactual explanations can clarify the decision-making process of black-box accident severity models and provide actionable insights. They can inform policy decisions, to identify the most valuable improvements to reduce accident severity, such as alternative junction types, improving street lighting, and implementing periodic driver retesting. By quantifying both global importance and regional variability, this approach enables more targeted interventions for policymakers and city planners.

Most of the data used to demonstrate the technique in this study are nominal, meaning the categories, such as $Types\ of\ Junction$ and $Vehicle\ Movement$ have no inherent order or numerical meaning.  Label encoding was used to convert categories into numerical values, yet this introduces an artificial order. This can bias distance-based nearest-neighbour and counterfactual generation approaches, leading to inaccurate assessments of feature similarity and undermining the reliability of the explanations. As such, further work is required to refine the implementation for ordinal features and must include collaboration with domain experts. Utilising techniques to causal reasoning and building on recent work in this domain \cite{srivastava2024road} would enable more robust conclusions to be drawn. Future work should also incorporate additional evaluation metrics for counterfactuals, especially those assessing sufficiency and necessity. Building on the framework from \cite{kommiya2021towards}, these metrics would assess whether certain features are essential to maintain the original prediction (sufficiency) and how their modification affects the outcome (necessity), providing further insights. 


%To enhance robustness and applicability, future research should include data from diverse geographic regions—across cities, countries, and climate zones—to capture variations in road conditions, traffic flow, and driving behavior.

%Additionally, relying solely on tabular data may miss critical context. Integrating multi-modal sources—such as traffic surveillance videos, vehicle sensors, GPS trajectories, and real-time traffic data—can provide a richer, more dynamic understanding of accidents and improve the accuracy and generalizability of counterfactual explanations.

 %Conditional probability-based metrics will enable more rigorous sensitivity analyses, helping to quantify the stability and relevance of input features in counterfactual scenarios.


Alongside input from domain experts and existing analytical techniques, the introduced framework provides a complimentary method to assist decision makers such as policymakers and city planners in efforts to reduce traffic accident severity and save lives.

%The majority of data used in this study are nominal data, which refers to data in which the categories have no inherent order or metric, such as $Types\ of\ Junctio$ and $Vehicle\ movement$. These categories are only used to represent different types or states and do not contain any quantitative or ordinal information. Traditional normalization methods, such as min-max scaling or standardization, are primarily designed for continuous numerical attributes or data with an inherent order, and therefore cannot be directly applied to nominal data. Although label encoding can be used to convert these categories into numerical values, this approach implicitly introduces an artificial order that does not reflect the actual similarities or differences among the categories. As a result, during the distance-based counterfactual generation process, such an unjustified order can lead to biases in the distance calculations, causing certain categories to be mistakenly evaluated as more dissimilar than they truly are. This bias ultimately impacts the accuracy of feature modification judgments and the objectivity of the explanation process, thereby undermining the effectiveness and reliability of the counterfactual explanation method.
\begin{comment}
The accident data used in this study were collected exclusively from Addis Ababa Sub-city between 2017 and 2020. This limited geographic and temporal scope means the dataset reflects only the specific local conditions—such as traffic patterns, driving behavior, infrastructure, climate, and safety regulations—which may differ substantially from those in other regions. For example, variations in road design, traffic volume, enforcement, and public transport across different cities or rural areas could significantly impact the model’s prediction and explanation performance elsewhere. The narrow time frame also limits the model’s ability to capture long-term trends or cyclical changes, reducing its generalizability.
\end{comment}
%To improve robustness and applicability, future research should incorporate data from diverse geographic regions—spanning different cities, countries, and climate zones—to account for broader variations in road conditions, traffic flow, and driving behavior. Expanding the dataset to cover a longer time period, including both recent and historical data, would help capture evolving traffic patterns. Moreover, relying solely on tabular data may overlook complex accident-related factors. Future studies should integrate multi-modal data such as traffic surveillance videos, vehicle sensors, GPS trajectories, and real-time traffic conditions. These additions can provide a more dynamic, comprehensive understanding of accidents and enhance the accuracy and generalizability of counterfactual explanations by giving the model a richer representation of real-world driving contexts.

%A promising direction for future work is to incorporate additional evaluation metrics for counterfactual explanations, particularly those assessing sufficiency and necessity. Building on the framework proposed by \cite{kommiya2021towards}, future studies will quantitatively evaluate whether key features are both necessary for, and sufficient to maintain, the original prediction. Metrics based on conditional probabilities will be adapted to assess feature relevance (sufficiency) and the effect of modifying features (necessity), enabling a more rigorous sensitivity analysis. This will help evaluate how small input or model changes influence counterfactual outcomes.

\begin{comment}
Although this study uses DiCE with a Random Forest model, future research should compare other counterfactual generation methods, such as WachterCF and newer algorithms that incorporate causal inference or graph-based techniques. Evaluating a variety of machine learning models—including logistic regression, multilayer perceptrons (MLPs), and other ensemble methods—will further test the generalizability and robustness of the counterfactual explanations across different architectures. This comparison will clarify how explanation quality is affected by the choice of model and counterfactual generation method.
\end{comment}

\begin{comment}
Future work should enlarge the geographic and temporal scope of the dataset, strengthen the causal validity and stability of generated counterfactuals, and investigate normalization strategies for nominal features. Integrating multi modal traffic data, applying necessity and sufficiency metrics, and exploring alternative generation methods promise to further enhance the reliability and utility of counterfactual explanations in traffic safety applications.
\end{comment}




==> SoGood_Workshop_Submission/sections/experimental.tex <==
\section{Experimental}
We demonstrate our proposed method on a dataset containing $12,316$ samples and $12$ features (Table \ref{tab:ft}), collected from traffic accident records of the Addis Ababa Sub-city Police Department during the years 2017 to 2020 \cite{endalie2023analysis}. The data was preprocessed by encoding text features and the dataset was then randomly divided into an $80\%$ training set and a $20\%$ test set. A random forest accident severity binary classification model was trained and performance assessed using accuracy and the F1 score. The target variable $(y)$, $Accident\ severity$, was composed of minor (low) and severe (high) severity accidents. Counterfactual explanations were generated using DiCE, going from severe accident severity factuals to counterfactuals in the minor accident severity class \cite{mothilal2020explaining}.\\

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    \textbf{Features} & \textbf{Number of Categories} & \textbf{Example Category} \\
    \hline
         $Age-band\ of\ driver$ & 5 & 31--50 \\
    \hline
         $Sex\ of\ driver$ & 3 & Male \\
    \hline             
         $Driving\ experience$ & 7 & 5--10yr \\
    \hline             
         $Types\ of\ Junction$ & 8 & Crossing \\
    \hline             
         $Road\ surface\ type$ & 6 & Asphalt roads \\
    \hline             
         $Light\ conditions$ & 4 & Darkness -- lights lit \\
    \hline             
         $Weather\ conditions$ & 9 & Raining \\
    \hline             
         $Type\ of\ collision$ & 10 & Rollover \\
    \hline             
         $Vehicle\ movement$ & 13 & Going straight \\
    \hline             
         $Pedestrian\ movement$ & 9 & Not a Pedestrian \\
    \hline
         $Cause\ of\ accident$ & 20 & Driving carelessly \\
    \hline                  
    \end{tabular}
    \caption{Summary of the 11 input features, showing the number of categories and an example for each. All features were nominal except for $Age-band\ of\ driver$ and $Driving\ experience$ which were ordinal.}
    \label{tab:ft}
\end{table}

\begin{comment}
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    Features & Number of Categories & Nominal/Ordinal \\
    \hline
         Age-band of driver & 5 & Ordinal \\
    \hline
         Sex of driver & 3 & Nominal \\
    \hline             
         Driving experience & 7 & Ordinal \\
    \hline             
         Types of Junction & 8 & Nominal \\
    \hline             
         Road surface type & 6 & Nominal \\
    \hline             
         Light conditions & 4 & Nominal \\
    \hline             
         Weather conditions & 9 & Nominal \\
    \hline             
         Type of collision & 10 & Nominal \\
    \hline             
         Vehicle movement & 13 & Nominal \\
    \hline             
         Pedestrian movement & 9 & Nominal \\
    \hline
         Cause of accident & 20 & Nominal \\
    \hline                  
    \end{tabular}
    \caption{Summary of the 11 input features, showing for each the number of categories and whether the feature is ordered.}
    \label{tab:ft}
\end{table}
\end{comment}
To adhere to the actionability of counterfactuals, $Age-band\ of\ driver$ and $Sex\ of\ driver$ were set as immutable features during the counterfactual generation process, as they are factors that cannot be altered in a real driving scenario. \par

For the global implementation, $N_{F} = 200$, and $N_{CF} = 10$ were utilised, meaning that 200 factual instances were randomly selected from across the severe accident class. For each factual, 10 counterfactuals in the low severity class were identified. For the regional analysis, for each of the four regions one factual instance which met a certain criteria (for example, high driving experience) was randomly selected and its four nearest neighbours which met the same selection criteria, resulting in $N_{F} = 5$ to form a region of five similar instances. As with the global approach, for each factual $N_{CF} = 10$ counterfactuals were identified for each. The average change frequency and standard deviation for each feature change were then calculated. Code implementing the technique for these experiments will be available upon publication\footnote{\url{https://github.com/anoynmous\_repo\_to\_share}}.


==> SoGood_Workshop_Submission/sections/limitations_future_work.tex <==
\section{Limitations}
\subsection{Dataset}
The accident record data used in this study were only collected from Addis Ababa Sub-city, and the data collection period is limited to 2017–2020. This geographical limitation means that the traffic accident cases included in the dataset only reflect the specific regional characteristics such as local traffic conditions, driving habits, road infrastructure, climate, and related safety management measures, which may differ significantly from those in other regions. For example, road design, traffic volume, enforcement intensity, and public transportation facilities in other cities or rural areas may vary considerably, potentially affecting the accident prediction and explanation performance of the same model when applied elsewhere. In addition, the limited time span of the data may prevent the study from capturing long-term trends or cyclical fluctuations in traffic accident patterns over time, thereby impacting the model's generalizability to scenarios beyond the historical data. In summary, these geographical and temporal limitations may result in the model performing less consistently in a broader range of application contexts, thereby affecting its generalizability and reliability.
\subsection{Uncertainty in Counterfactual Generation}
The study primarily relies on the DiCE algorithm to generate counterfactual explanations. Although the algorithm performs exceptionally well in maintaining the sparsity and feasibility of counterfactual explanations, allowing the model's prediction to be changed through relatively few feature modifications, the generated results may in some cases fail to truly capture the causal relationships between variables. In other words, while adjusting certain input features can change the model’s prediction, such changes may not necessarily reflect the actual causal mechanisms, and may therefore differ from the true causal effects.

Moreover, the stability of the generated counterfactual results faces significant challenges. Since the generation process is highly dependent on the initial state of the input data and the model parameters, its outcomes can be affected by several factors. First, the influence of input perturbations on the results is not negligible, as even minor data noise or slight perturbations may lead to substantial changes in the generated counterfactual instances, thereby reducing the robustness of the explanations. Second, as the model undergoes updates or retraining, changes in the internal decision boundaries may render previously generated counterfactual explanations ineffective, which can compromise the consistency of the interpretations. Finally, the algorithm's hyperparameters are highly sensitive in the counterfactual generation process; different settings may result in significant variations in minimizing feature modifications or ensuring the diversity of the generated counterfactuals, ultimately causing the final explanation results to exhibit instability across repeated experiments.



\subsection{Inability to Effectively Normalize Nominal Categorical Data}
The majority of data used in this study are nominal data, which refers to data in which the categories have no inherent order or metric, such as $Types\ of\ Junctio$ and $Vehicle\ movement$. These categories are only used to represent different types or states and do not contain any quantitative or ordinal information. Traditional normalization methods, such as min-max scaling or standardization, are primarily designed for continuous numerical attributes or data with an inherent order, and therefore cannot be directly applied to nominal data. Although label encoding can be used to convert these categories into numerical values, this approach implicitly introduces an artificial order that does not reflect the actual similarities or differences among the categories. As a result, during the distance-based counterfactual generation process, such an unjustified order can lead to biases in the distance calculations, causing certain categories to be mistakenly evaluated as more dissimilar than they truly are. This bias ultimately impacts the accuracy of feature modification judgments and the objectivity of the explanation process, thereby undermining the effectiveness and reliability of the counterfactual explanation method.


\section{Future Work}
\subsection{Data expansion and diversity enhancement}
Future research could consider collecting traffic accident data from a broader range of geographical areas, including different cities, countries, and even regions with varied climate zones, in order to capture a more diverse range of road structures, traffic flows, driving behaviors, and environmental factors. Additionally, the data collection period should be extended in the time dimension to include not only recent accident data but also historical data, thereby more comprehensively reflecting the long-term trends and changes in traffic accidents. In terms of data diversity, relying solely on text or numerical data may not be sufficient to reveal all the complex factors underlying traffic accidents. Thus, future work should actively incorporate multi-modal data, such as traffic surveillance videos, vehicle sensor data, GPS trajectories, and other real-time data related to the traffic environment, to understand the dynamic processes and potential causal relationships behind accidents from multiple perspectives, thereby improving the accuracy and practical applicability of counterfactual explanations. By combining the visual information from video images with the real-time dynamics of sensor data, the model can obtain a more comprehensive representation during training, thereby enhancing its robustness and generalization capabilities.
\subsection{Evaluation Metrics – Necessity and Sufficiency}
One promising direction is to incorporate and investigate additional evaluation metrics for counterfactual explanations, particularly focusing on sufficiency and necessity. Inspired by the framework proposed in \cite{kommiya2021towards}, future work will quantitatively assess whether the key features identified are both necessary for, and sufficient to maintain, the original predictions. By adapting metrics that capture the conditional probability of feature relevance (sufficiency) and the impact of feature modification (necessity), we aim to provide a more robust sensitivity analysis of the explanations. This sensitivity study would evaluate how small perturbations in the input or model parameters affect the counterfactual outcomes.

\subsection{ Exploring Alternative Counterfactual Generation Methods and Machine Learning Models}
While the current work utilizes DiCE with a Random Forest model, it would be beneficial to compare the performance and stability of different counterfactual generation approaches. Future studies will evaluate alternative methods such as WachterCF and newer algorithms that may integrate causal inference or graph based techniques. In addition, applying different machine learning models, ranging from simpler logistic regression and multilayer perceptrons (MLP) to other ensemble methods, will help determine the generalizability and robustness of the counterfactual explanations under various modeling paradigms. This exploration is expected to shed light on the sensitivity of the explanation quality when the underlying model architecture changes.

==> SoGood_Workshop_Submission/sections/method.tex <==
\section{Method - Feature Change Frequency}
Feature change frequency can serve as a key metric for evaluating the importance of features in counterfactual explanations. It is defined as the proportion of times a feature is changed between factual instances (high severity accidents) and identified counterfactual instances (low severity accidents). The change frequency of feature $j$  of an instance $i$ for $N_{CF}$ counterfactual samples is given by: 
\begin{equation}\label{eq:local}
    f_j^{instance}(i)=\frac{1}{N_{C F}} \sum_{k=1}^{N_{C F}} I\left(X_{j}(i, k) \neq X_{j}(i, \text { orig })\right)
\end{equation}
where 
\begin{equation}\label{eqn:6}
    I\left(X_{j}(i, k) \neq X_{j}(i, \text { orig })\right)=\left\{\begin{array}{ll}
1, & \text { if } X_{j}(i, k) \neq X_{j}(i, \text { orig })  \\
0, & \text { otherwise }
\end{array}\right.
\end{equation}
For the $i^{th}$ sample, let the original value of feature $X_j$ be denoted as $X_j(i,orig)$ , and let the value in the $k^{th}$ counterfactual instance of the $i^{th}$ sample be denoted as $X_j(i,k)$. By comparing $X_j(i,k)$ with $X_j(i,orig)$, using an indicator function $I(\cdot)$ that returns $1$ if the values differ and $0$ otherwise as shown in Eqn \ref{eqn:6}, it is recorded whether the feature changes in each counterfactual instance. 
%The inner summation $\sum_{k=1}^{n_{C F}}$ iterates over all counterfactual instances for each sample.
The hypothesis is that if a feature is frequently modified in counterfactual instances, it may play an important role in altering the model’s prediction; conversely, if a feature is seldom changed, the feature may not have a large influence on the classification outcome. This frequency metric can be applied to find both global and regional feature importances (Fig \ref{fig:methods_fig}).

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{SoGood_Workshop_Submission/figures/2d_method_5.png}
    \caption{Method demonstrated for a toy 2D dataset. 1) Train a binary classifier for accident severity 2) Select individual factual instances (yellow marker) from the high severity class, and identify nearby datapoints in the low severity class (counterfactuals, lilac marker), shown here for $N_{CF} = 3$ counterfactuals. 3) In the regional case, around a selected instance (yellow marker) select N nearest neighbours (shown here with green and pink bounds for two regions A and B) and identify corresponding counterfactuals (lilac marker). 4) To generate global insights, randomly select a high number of factual datapoints (yellow marker) across the data space, and identify corresponding counterfactuals in the low severity class (lilac marker). For all scenarios, feature change frequency is calculated as described to quantify how frequently feature values change between selected factuals and counterfactuals.}
    \label{fig:methods_fig}
\end{figure}

\subsection{Global and Regional Feature Change Frequency}
In the global feature importance, the overall modification frequency of each feature is determined by statistically analyzing counterfactual instances generated for each sample across the dataset, thereby identifying the key features that consistently drive prediction changes. 
Regional feature importance is found by choosing a query factual and identifying the most similar samples to the query factual to form a region and then generating counterfactuals for all the samples in the region. A nearest neighbor algorithm using the Hamming distance is used to identify the samples most similar to the given query sample, wheere Hamming distance is defined as:
\begin{equation}
    d_h(x,y)=\sum_{j=1}^{m}I(x_j\neq y_j)
\end{equation}
Within this target region, the modification frequency of each feature is computed from the counterfactual instances, and the average and standard deviation of these local modification frequencies are further calculated.
The global and regional feature change frequency can be calculated using a generic formula of $F_j$ for feature $X_j$ using the following formula:


\begin{equation}\label{eq:regional}
    F_{j}=\frac{1}{N_{F}} \sum_{i=1}^{N_{F}} f_j^{instance}(i) 
\end{equation}
where global frequency $F^{global}_{j}$, and regional frequency, $F^{Region}_{j}$, may use different values for 
$N_{F}$ and $N_{CF}$ given the differing magnitude of datapoints they each represent.

\begin{comment}
    

\begin{equation}
    \sigma_{f_j^{local}}=\sqrt{\frac{1}{N}\sum_{i=1}^{N}(f_j^{local}(i)-\overline{f_j^{re}})^2}
\end{equation}


\begin{equation}
    F_{j}=\frac{1}{N \times n_{C F}} \sum_{i=1}^{N} \sum_{k=1}^{n_{C F}} I\left(X_{j}(i, k) \neq X_{j}(i, \text { orig })\right)
\end{equation}
\end{comment}
%Suppose there are $N_{F}$ samples, and for each sample, $N_{CF}$ counterfactuals are generated.  and the outer summation $\sum_{i=1}^{N}$ iterates over all samples.



\begin{comment}
\begin{equation}
    \overline{f_j^{re}}=\frac{1}{N}\sum_{i=1}^{N}f_j^{local}(i)
\end{equation}


$\overline{f_j^{re}}$ represents the mean local change frequency of feature $j$ across all samples, $N$  denotes the total number of samples considered, and $f_j^{local}(i)$ represents the local change frequency of feature $j$ for the $i$th sample in this region.

\begin{equation}
    \sigma_{f_j^{local}}=\sqrt{\frac{1}{N}\sum_{i=1}^{N}(f_j^{local}(i)-\overline{f_j^{re}})^2}
\end{equation}
\end{comment}
%$\sigma_{f_j^{local}}$ denotes the standard deviation of the local change frequency of feature $j$, which measures the variability of this frequency across different samples.


\subsection{Assessing Regional Feature Distribution Changes}
To assess how individual features behave within a given sample and its corresponding regional group compared to the generated counterfactuals, we employ a mode-based statistical method. 

First, for each feature, we identify the most common category (i.e., the mode) and calculate its proportion within the factual data points. This provides a baseline for the primary distribution of that feature. We then analyze how this distribution changes in the corresponding counterfactual instances by calculating the proportion of the same mode within the counterfactual data.

By comparing these proportions, we can observe whether and to what extent the mode's prevalence changes during counterfactual generation. This change is quantified using the relative change rate, defined as:
\begin{equation}\label{eq:rc}
    \delta_j=\frac{p_j^{cf}-p_j^{orig}}{p_j^{orig}}
\end{equation}
where $p_j^{orig}$ is the proportion of the most common category for feature $j$ in the factual sample, and $p_j^{cf}$ denotes the proportion of the same category in the counterfactuals. The metric $\delta_j$ quantifies the percentage change in the proportion of that category during the counterfactual generation process and provides a standardized measure. If $\delta_j$ is positive, it indicates that the proportion of that category has increased in the counterfactual data; if negative, the proportion has decreased.

When $|\delta_j|$ is small, it indicates that the counterfactual generation process has little impact on the main distribution of that feature, demonstrating that the local explanation is relatively stable and consistent with respect to that feature. Conversely, when $|\delta_j|$ is large, it suggests that significant shifts occur in that feature during the counterfactual generation process, which may imply that the feature plays a more critical role in the regional explanation.

\subsection{Correlation Analysis of Regional and Global Change Frequencies}
We calculate the correlation between the regional and global feature change frequencies in order to understand if different regions are affected predominantly by global behaviour or region-specific behaviour. The correlation between the regional $F_j^{region}$ and the global change frequency $F_j^{global}$, is calculated using the Pearson correlation coefficient (PCC) as follows:
\begin{equation}
    r=\frac{\sum_{j=1}^{m}(F_j^{region}-\mu_{re})(F_j^{global}-\mu_{g})}{\sqrt{\sum_{j=1}^{m}(F_j^{region}-\mu_{re})^2}\sqrt{\sum_{j=1}^{m}(F_j^{global}-\mu_{g})^2}}
\end{equation}
where $\mu_{re}$ and $\mu_{g}$ represents the mean regional and global feature change frequencies respectively.

In Fig \ref{fig:egr}, the example points A, B, C, and D are illustrate different feature correlation scenarios, where the line y = x, represents equal global and regional importance of a particular feature. Therefore, the distance of a data point from this line reflects the degree of consistency or deviation between its global and regional importance.

Point A represents data in the upper-left quadrant, where the feature exhibits low global feature importance but high regional feature importance. This indicates that while the feature does not significantly impact the overall model predictions, it is very important for defining the accident severity classification of samples in this data region. 

Point B represents data in the lower-left quadrant, where the feature neither stands out on a global scale nor exhibits exceptional prominence regional, suggesting that its influence on model predictions remains low both globally and regionally. 

Point C represents data in the upper-right quadrant, where the feature has high importance in both global and regional dimensions, signifying that it plays a crucial role not only in the overall dataset but also within specific localised samples. 

Point D represents data in the lower-right quadrant, where the feature shows high global importance but is not prominent regionally, indicating that, although it has a significant impact on overall model predictions, its importance does not manifest in some individual samples or regions. 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{SoGood_Workshop_Submission/figures/egr.png}
    \caption{Example points A, B, C, and D are for illustration only: A indicates low global but high regional importance; B shows both are low; C indicates both are high; and D shows high global but low regional importance. The distance of each point from the line y = x reflects the consistency or deviation between global and regional importance.}
    \label{fig:egr}
\end{figure}


==> SoGood_Workshop_Submission/sections/related_work.tex <==
\section{Related work}
The application of artificial intelligence (AI) techniques to predict traffic accident severity has gained significant attention in traffic safety research. Models based on artificial neural networks have shown promise in extracting informative features from multidimensional traffic data for severity prediction \cite{hamdan2023traffic}. Several studies have identified key influencing factors such as speed, weather, and road conditions through machine learning and deep learning approaches \cite{siswanto2023artificial}. Others have employed SHAP to interpret the influence of variables like speeding and road category on accident fatality rates \cite{panda2023predicting}. Combining state-of-the-art deep learning models with explainable AI (XAI) methods has further enhanced model transparency by quantifying the contribution of various features \cite{aboulola2024automated}. From a risk analysis standpoint, models such as XGBoost, Random Forest, and deep neural networks have been integrated with SHAP to provide interpretable insights into how driver behavior and environmental conditions affect injury severity \cite{abdulrashid2024explainable}. Counterfactual explanations have also been used for traffic accident prediction such as the work by Artelt et al where the use of multi-instance counterfactuals enable global analysis by generating improvement strategies for groups of accidents, rather than isolated cases \cite{artelt2021application}.

Our work is closely related to approaches that integrate counterfactual explanations with feature importance analysis. For instance, Meulemeester et al. \cite{meulemeester2023calculating} propose incrementally modifying features from factual to counterfactual values to quantify their contribution to prediction changes, effectively linking counterfactuals with SHAP values. Most similar to our work is the method by Mothilal et al. \cite{kommiya2021towards}, which generates counterfactuals for individual instances and derives importance scores based on which features change or remain constant. While their approach emphasizes interpretability on an instance level, our work extends this idea by focusing on regional and global feature importance, offering broader insights across groups of accident scenarios.






\begin{comment}
The use of artificial intelligence (AI) techniques to directly predict or analyse traffic accident severity has become an important research direction in the field of traffic safety, including the use of artificial neural networks \cite{hamdan2023traffic}. By using machine learning and deep learning models, effective features can be extracted from multidimensional traffic data to predict and explain accident severity. The problem of traffic accident prediction was explored using AI models and it was observed that factors such as speed, weather, and road conditions have a significant influence in prediction \cite{siswanto2023artificial}. Other studies have utilised the SHAP method on prediction models, identifying the role of key variables such as speeding and road category on accident fatality rates \cite{panda2023predicting}. In addition, research using state of the art deep learning architectures in combination with explanatory AI techniques has further improved the transparency and reliability of the prediction models by quantitatively analysing the contribution of multiple features \cite{aboulola2024automated}. From a risk analysis perspective, XGBoost, Random Forest and Deep Neural Networks were integrated and SHAP values were used to reveal the impact of driving behaviour and environmental factors on injury severity, providing a more intuitive basis for decision-making \cite{abdulrashid2024explainable}.\par

Compared to other XAI methods, the counterfactual approach has the following advantages in traffic accident prediction; firstly, it can provide explicit and actionable suggestions to transform model-predicted severe accidents into non-severe ones; secondly, through multi-instance counterfactual interpretation, the approach is able to generate global improvement proposals for a group of accident cases simultaneously, instead of limiting itself to a single case, thus better capturing group characteristics ; moreover, the method improves the interpretability of the black-box model by ensuring the feasibility and cost-effectiveness of the recommendations while minimising attribute changes \cite{artelt2021application}.


Similar to our work, there are different approaches which integrate counterfactual explanations with feature importances. This generally involved observing how feature changes contributed to the change in model prediction score, we can change these features from the factual to the counterfactual value one by one, each time evaluating the difference in the model outcome. This can be used to generate SHAP scores for the different features \cite{meulemeester2023calculating}.
Our work is most similar to the work by Mothilal et al \cite{kommiya2021towards}, which genearates feature importance scores by gneerating a set of counterfactuals for a single example and examining how the feautrs change for a single data point, and using the examining which features stay the same and which feautres change and translaiting thse for metrics of sufficiency of neccessity whihc is used to provide a counterfactual; score. this is similar to our approach as we also look at how the feautrs of a counterfactuals change, though our work takes focuses more on looking at the importance of feautres in a regional or global scale rather than a local scale as in the work done by Mothilal et al \cite{kommiya2021towards}.
\end{comment}

==> SoGood_Workshop_Submission/sections/results_and_discussion.tex <==
\section{Result and Discussion}
\label{section:results}
%\subsection{General performance}
The trained model had an F1 score of $79\%$ and accuracy of $83.47\%$ on the test set, which is comparable to other ML models that have F1 scores between $77$ to $86\%$ and accuracies between $70$ to $85\%$ \cite{endalie2023analysis}. Therefore we deemed our model to be sufficient for effective counterfactual generation. DiCE resulted in sparse feature changes in the generated counterfactuals, with the majority of counterfactuals changing two or fewer features values (1460 instances of 2000, 70.3\%). Such concise explanations are both interpretable and practical, reflecting real-world constraints where only a few factors can reasonably be adjusted. Sparse counterfactuals thus enhance usability and support targeted interventions in accident prevention.

\begin{comment}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{SoGood_Workshop_Submission/figures/global_sparsity.pdf}
    \caption{ Distribution of the number of modified features in counterfactual instances generated from $2000$ factual cases, with modifications ranging from one to seven features.}
    \label{fig:xishu}
\end{figure}





In the global feature modification sparsity analysis, the figure \ref{fig:xishu} shows the distribution of the number of modified features across all counterfactual instances: the counterfactual with two modified features is the most frequent, with $1216$ instances; 338 instances have three modified features, while $230$ instances have only one modified feature; the numbers of instances for four, five, six, and seven modified features are $104$, $60$, $30$, and $22$, respectively. This indicates that in most counterfactual instances, only a relatively small number of features are modified, primarily concentrated in the range of one to three features.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{SoGood_Workshop_Submission/figures/xishu.png}
    \caption{ Distribution of the number of modified features in counterfactual instances generated from $2000$ factual cases, with modifications ranging from one to seven features.}
    \label{fig:xishu}
\end{figure}


This model exhibits good sparsity as most counterfactual instances require only modifying one to three features to change the prediction from ``severe" to ``non-severe". This not only makes the explanation more intuitive but also aligns with real-world scenarios, where users or decision-makers typically can only adjust a limited number of controllable factors. Sparse and clear explanations can better guide practical interventions, thereby enhancing the operability of accident prevention measures.
\end{comment}
\begin{comment}
To evaluate the sparsity of the counterfactual explanations, in the global explanation stage, each counterfactual instance is compared with its corresponding original sample one by one using the indicator function \eqref{eq:6} to determine whether each feature has changed, and the number of changed features is calculated for each counterfactual instance. Then, the change counts for all counterfactual instances are aggregated to obtain the global distribution of feature changes.

Figure \ref{fig:xishu} shows the distribution of the number of modified features across all counterfactual instances. The most common case involves two feature changes (1,216 instances), followed by three (338 instances) and one (230 instances). Fewer instances involve four (104), five (60), six (30), or seven (22) feature modifications. This indicates that most counterfactuals require only one to three feature changes.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{SoGood_Workshop_Submission/figures/xishu.png}
    \caption{ Distribution of the number of modified features in counterfactual instances generated from $2000$ factual cases, with modifications ranging from one to seven features.}
    \label{fig:xishu}
\end{figure}

The model demonstrates strong sparsity, as minimal modifications are typically sufficient to flip a prediction from "severe" to "non-severe." Such concise explanations are both interpretable and practical, reflecting real-world constraints where only a few factors can be adjusted. Sparse counterfactuals thus enhance usability and support targeted interventions in accident prevention.
\end{comment}

\begin{comment}
\section{Counterfactual Explanation}
For the randomly selected factual instance labeled “severe,” five counterfactual instances were generated, each configured to exhibit a “non severe” accident severity outcome. In each counterfactual, one or two features are modified, causing the accident severity to change to ``non-severe". Figure \ref{fig:tezheng} displays the feature modifications in these five counterfactual explanations.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{SoGood_Workshop_Submission/figures/tezheng.png}
    \caption{Five generated counterfactuals for reducing accident severity from “severe” to “non-severe”.}
    \label{fig:tezheng}
\end{figure}
\section{Feature Change Frequency}
\subsection{Global Feature Change Frequency }

In the figure \ref{fig:gl}, the horizontal axis represents the features, while the vertical axis shows the corresponding average change frequency ranging from $0$ to $1$. Specifically, the change frequency for $Cause\ of\ accident$ is $0.38$, the highest among all features; $Driving\ experience$ follows at $0.376$; $Type\ of\ collision$ is $0.26$; $Vehicle\ movement$ is $0.228$; $Weather\ conditions$ is $0.196$; $Types\ of\ Junction$ is $0.192$; $Light\ conditions$ is $0.164$; $Pedestrian\ movement$ is $0.148$; and $Road\ surface\ type$ is $0.136$.
\end{comment}

\subsection{Global Feature Change Frequency }
We look at the global feature change frequency of different features to see which features were globally the most important for accident severity classification.
A total of $N_F = 200$ factual instances were selected, and for each instance $N_{CF} = 10$ counterfactuals were generated to calculate the global feature change frequency (where the value varies between 0 to 1) to rank the features in terms of importance, which is presented in Table \ref{tab:feature_importance}.


\begin{table}[h!]
\centering
\begin{tabular}{|c|l|c|}
\hline
\textbf{Rank} & \textbf{Feature} & \textbf{Mean Change Frequency} \\
\hline
1 & $Driving\ experience$ & 0.337 ± 0.238 \\
\hline
2 & $Cause\ of\ accident$ & 0.331 ± 0.226 \\
\hline
3 & $Type\ of\ Junction$ & 0.289 ± 0.242 \\
\hline
4 & $Type\ of\ collision$ & 0.279 ± 0.217 \\
\hline
5 & $Vehicle\ movement$ & 0.233 ± 0.221 \\
\hline
6 & $Weather\ conditions$ & 0.223 ± 0.215 \\
\hline
7 & $Pedestrian\ movement$& 0.216 ± 0.169 \\
\hline
8 & $Light\ conditions$ & 0.203 ± 0.211 \\
\hline
9 & $Road\ surface\ type$ & 0.103 ± 0.126 \\
\hline
\end{tabular}
\caption{Global feature importance ranking based on mean change frequency with standard deviation. A higher change frequency demonstrates increased importance of the corresponding feature in producing counterfactuals.}
\label{tab:feature_importance}
\end{table}



\begin{comment}
\begin{table}[htbp]
\centering
\begin{tabular}{|c|c|c|}

\hline
Rank & Feature              & Change Frequency \\
\hline

1    & Cause of accident   & 0.38           \\
\hline
2    &Driving experience    & 0.367            \\
\hline
3    &Type of collision    & 0.26           \\
\hline
4    & Vehicle movement    & 0.228            \\
\hline
5    & Weather conditions  & 0.196             \\
\hline
6    & Types of Junction     & 0.192             \\
\hline
7    & Light conditions   & 0.164          \\
\hline
8    & Pedestrian movement     & 0.148         \\
\hline
9    & Road surface type    & 0.136            \\
\hline

\end{tabular}

\caption{Feature importance ranking based on change frequency}
\label{tab:feature_importance}
\end{table}
\end{comment}

\begin{comment}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{SoGood_Workshop_Submission/figures/gl.png}
    \caption{Global Feature Change Frequency in Counterfactual Generation from 2000 Factual Instances.}
    \label{fig:gl}
\end{figure}
\end{comment}


The high change frequencies for  $Driving\ experience$, $Cause\ of\ accident$ and $Types\ of\ Junction$ indicate that these three features are adjusted most often to change a “severe” prediction to a “minor” accident severity prediction. %Knowing these, a driver with low $Driving\ experience$ (inexperienced) should be aware of particular accident causes and junction types to prevent high-severity accidents from occurring.
This aligns with previous work, which found roadway design and speed-related factors dominant via SHAP \cite{aboulola2024improving}, and another which flagged the importance of junction type \cite{wang2024prediction}.


The least importance features were $Light\ conditions$ and $Road\ surface\ type$. This showed that the presence of pedestrians or surface of the road is unlikely to make a large difference to the severity of the collision compared to the other features considered by the model.
The high standard deviation of the values across all features suggest inconsistencies in the feature importance across samples and is highly dependent on the context/ region we consider, therefore motivating a regional approach.

\begin{comment}
Moderate modification frequencies for $Type\ of\ collision$ and $Vehicle\ movement$ further highlight their influence on the model’s decisions. Intermediate change frequencies for $Weather\ conditions$, $Types\ of\ Junction$ and $Light\ conditions$ (0.164) show a secondary level of importance, while the lower frequencies for $Pedestrian\ movement$ and $Road\ surface\ type$ imply these features play a smaller role in counterfactual generation. Overall, this distribution of change frequencies reflects the degree to which the model relies on each feature when seeking minimal adjustments to alter its prediction. 
\end{comment}

\subsection{Regional Feature Change Frequency}
\begin{comment}
A single factual instance was randomly selected, and its five nearest neighbors were identified to form a region consisting of six factual instances. For each instance, $10$ counterfactuals were generated. 
In the local feature frequency, the average change frequency and standard deviation for each feature were computed separately for six regions, shows in figures \ref{fig:overall}.
In Region $1$ figure \ref{fig:local1}, the average change frequency of $Driving\ experience$ is 0.23 (Std = 0.18), $Types\ of\ Junction$ is $0.43$ (Std = $0.21$), and $Type\ of\ collision$ is $0.43$ (Std = $0.29$). $Road\ surface \ type$ remains $0$ throughout this region, indicating that this feature was not modified at all. This pattern suggests that the counterfactual modifications in Region 1 predominantly focus on adjusting the features related to junction types and collision types, which are modified most frequently, while the driving experience is changed less often, and the road surface type plays no role in altering the prediction.


In Region $2$ figure \ref{fig:local2}, the value for $Type\ of\ collision$ is $0.53$; in Region $3$ figure \ref{fig:local3}, $Types\ of\ Junction$ and $Light\ conditions$ have values of $0.47$ and $0.2$7 respectively, while $Pedestrian\ movement$ is only $0.03$; in Region $4$ figure \ref{fig:local4}, both $Types\ of\ Junction$ and $Light\ conditions$ are likewise $0.47$ and $0.27$ respectively, and $Vehicle\ movement$ is $0.30$.

In Region $5$ figure \ref{fig:local5}, the average change frequency for $Types\ of\ Junction$ is significantly high at 0.56 (Std = 0.21), while the change in $Light\ Conditions$ is very small, at only 0.05 (Std = 0.03). In Region 6 figure \ref{fig:local6}, $Driving\ Experience$ remains high, with an average change frequency of 0.44 (Std = 0.17); however, $Types\ of\ Junction$ significantly drops to 0.25 (Std = 0.17), and $Road\ Surface\ Type$ remains extremely low at only 0.04 (Std = 0.02). The modification frequency for $Type\ of\ Collision$ increases to 0.42 (Std = 0.26), indicating a more significant impact on decision changes.



\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{chapters/chapter04/local1.png}
    \caption{Region 1}
    \label{fig:local1}
  \end{subfigure}%
  \hspace{0.5cm}
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{chapters/chapter04/local2.png}
    \caption{Region 2}
    \label{fig:local2}
  \end{subfigure}

  \vspace{0.7cm}
  
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{chapters/chapter04/local3.png}
    \caption{Region 3}
    \label{fig:local3}
  \end{subfigure}%
  \hspace{0.5cm}
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{chapters/chapter04/local4.png}
    \caption{Region 4}
    \label{fig:local4}
  \end{subfigure}
  \vspace{0.7cm}
  
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{chapters/chapter04/local5.png}
    \caption{Region 5}
    \label{fig:local5}
  \end{subfigure}%
  \hspace{0.5cm}
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{chapters/chapter04/local6.png}
    \caption{Region 6}
    \label{fig:local6}
  \end{subfigure}
  
\caption{Mean and standard deviation of local feature change frequencies computed for six regions, each formed by a randomly selected factual instance and its five nearest neighbors with $10$ counterfactuals generated per instance.}
\label{fig:overall}
\end{figure}

In Region $1$ and $2$, counterfactual explanations mainly rely on adjusting $Types\ of\ 
Junction$ and $Type\ of\ collision$, while $Road\ surface\ type$ remains unchanged in both regions, indicating that no modifications are made to pavement-related factors. In Region $2$, compared to Region $1$, the change frequency for $Type\ of\ collision$ is significantly higher, demonstrating a greater emphasis on adjustments related to collision type in that region. Both Region $3$ and Region $4$ exhibit a strong tendency to adjust $Types\ of\ Junction$ and $Light\ conditions$; however, in Region $3$, $Weather\ conditions$ are not modified at all and changes in $Pedestrian\ movement$ are minimal, whereas Region $4$ further incorporates adjustments to $Vehicle\ movement$ and $Cause\ of\ accident$, indicating some differences in local feature modifications between the two regions. 
Region $5$ displays a distinctly different pattern from the aforementioned regions, with counterfactual explanations tending to adjust $Road\ surface\ type$ and $Weather\ conditions$, which are directly related to the road and environmental factors, and a relatively lower reliance on $Driving\ experience$ and $Type\ of\ collision$. In Region $6$, the counterfactual modifications are primarily focused on $Driving\ experience$ and $Types\ of\ junction$, while the other features, especially $Cause\ of\ accident$, remain nearly stable, indicating that the changes in this region are mainly driven by driving behavior and junction types.
These differences reflect significant variations in the emphasis the model places on different features when generating counterfactual explanations across these six regions, stemming from the varying feature distributions or characteristics of the sample groups in each region.
\end{comment}

In addition to considering the global importance of features across the entire data space, certain features may be important in a particular context for accident severity. Therefore, we propose to explore the change frequency in local regions. We demonstrate this for regional approach for factuals chosen using contrasting feature categories for two features: the number of years of driving experience ($Driving\ experience$, <1 year and >10 years) and $Weather\ conditions$ ("normal" and "rainy"), resulting in four regions (Fig \ref{fig:overall}).

\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{SoGood_Workshop_Submission/figures/local_Driving_experience_3.pdf}
    \caption{Region 1: Driving\_experience >10 years}
    \label{fig:local1}
  \end{subfigure}%
  \hspace{0.5cm}
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{SoGood_Workshop_Submission/figures/local_Driving_experience_4.pdf}
    \caption{Region 2: Driving\_experience <1 year}
    \label{fig:local2}
  \end{subfigure}

  \vspace{0.7cm}
  
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{SoGood_Workshop_Submission/figures/local_Weather_conditions_4_rainy.pdf}
    \caption{Region 3: Weather\_conditions  = "rainy"}
    \label{fig:local3}
  \end{subfigure}%
  \hspace{0.5cm}
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{SoGood_Workshop_Submission/figures/local_Weather_conditions_2_normal.pdf}
    \caption{Region 4: Weather\_conditions  = "normal"}
    \label{fig:local4}
  \end{subfigure}
  
\caption{Mean and standard deviation of local feature change frequencies computed for four  contrastive regions, each formed by randomly selecting a factual instance and its four nearest factual neighbors with a specific categorical feature value (for example driving experience more than 10 years for region 1) and using $10$ counterfactuals generated per factual instance.}
\label{fig:overall}
\end{figure}


In Region 1 (Fig \ref{fig:local1}), representing a sample of highly experienced drivers, a change in the vehicle movement category was the largest contributor to reducing accident severity. The features suggested to be least important in influencing a reduction in accident severity were the road surface type and the weather conditions.

Region 2 (Fig \ref{fig:local2}) represents a region of inexperienced drivers. For this region, the lack of driving experience itself was found to be the most important feature in changing the accident severity from severe to minor. The \textit{Type of Junction}, \textit{Weather conditions} and \textit{Pedestrian movement} were all found to also be important features. In contrast to the experienced drivers of Region 1, the \textit{Vehicle movement} was consistently one of the least important features in reducing accident severity.

Regions 3 and 4  demonstrate the approach for differing weather conditions: "rainy" and "normal" respectively. For the factual instances presented in Region 3 (Fig \ref{fig:local3}), the \textit{Weather conditions} themselves ("rainy") were one of the largest accident severity contributors, followed by features including the \textit{Driving experience}: suggesting that sufficient driving experience is required in suboptimal weather conditions. Weather’s elevated importance under rainy conditions echoes results from a study into older-pedestrian crashes, where precipitation amplified risk factors that were muted in global models \cite{akter2025analyzing}. City planners could address this risk by investing in better road drainage and ensuring proper road markings. In contrast, for Region 4 (Fig \ref{fig:local4}), the "normal" weather conditions had a low impact on accident severity and the specific cause of the accidents were most important.

These results reveal clear regional variation in the features that drive counterfactual changes in the accident severity. These differences reflect nuanced underlying variations in the feature distributions and local dynamics of each region, highlighting the value of regional analysis.

For all four regions \textit{Road surface type} was consistently one of the least important features, correlating with the global finding (Table \ref{tab:feature_importance}). Similarities and differences between the regional and global importance are considered in more detail in a following section.








\subsubsection{Feature change insights for Region 1}
To demonstrate the potential to obtain more in-depth insights into the reason for severe accidents, we have performed further analysis for Region 1 (high \textit{Driving experience}) by considering the specific categorical feature values between factual and counterfactual instances.

Table \ref{tab:mode_comparison} compares the original factual samples from Region 1 with their counterfactuals, focusing on the most common categorical feature values (the mode). The reduction in mode frequency for each feature is represented by $\delta_j$. Given the default weighting that DiCE puts on enforcing sparsity when finding counterfactuals, as discussed typically only one or two feature values changed between factual and counterfactual instances.

For the case of Region 1, the high factual mode \% for most features indicates that our regional approach successfully identified groups of similar accident situations. For this region, \textit{Vehicle movement} was the largest contributor to accident severity. In the factual instances (severe accident severity), "Turnover" was the most frequent category, represented by 60\% of factual instances, suggesting that this is a common cause of severe accidents. In the counterfactual instances, the frequency of "Turnover" dropped to 14\% and instead the most common \textit{Vehicle movement} category in the minor accident severity group was "Going straight".

A more modest drop in occurrence of the most frequent feature categories occurred for the other features and the mode in the counterfactuals remained the same as for the factual instances, suggesting that they were modified only for a small number of instances and that these feature changes were less consistently important. \textit{Weather conditions}, \textit{Road surface type}, and \textit{Cause of accident} shows minimal change suggesting they have little influence on prediction outcomes and appear largely irrelevant in the counterfactual generation process. The change in frequency of the driving experience for this group of experienced drivers (100\% to 58\%) is quite surprising as it suggests that a driver having less experience would lower accident severity. A possible reason could be overconfidence in driving ability. To address this, drivers could be retested several years after obtaining their license to prevent complacency.

Further work is required, including involvement of domain experts, before drawing robust conclusions yet these initial findings reinforce the potential value of localised counterfactual analysis in uncovering key decision-driving factors within specific regions. The proposed method offers quantifiable insights that may be useful as part of wider analysis with domain experts.

\begin{comment}
Summary:
The analysis highlights that in Region 1, Type of Collision is the most influential feature in shifting predictions, followed by Types of Junction. Features like Weather Conditions and Road Surface Type appear largely irrelevant in the counterfactual generation process. These findings reinforce the value of localized counterfactual analysis in uncovering key decision-driving factors within specific regions.
\end{comment}
\begin{comment}
Type of Collision exhibits the largest shift, with a $\delta_j$ of –0.55. This substantial drop in the dominant category “Vehicle with vehicle collision” suggests it is a key factor influencing the prediction shift from “severe” to “non-severe,” aligning with its high change frequency in Region 1.

Types of Junction also shows a notable change ($|\delta_j| = 0.28$), but its impact is less pronounced, indicating the dominant category “Crossing” plays a secondary role in driving prediction changes.

In contrast, Weather Conditions and Road Surface Type show minimal or no change ($|\delta_j| = 0.017$ and $0.00$), suggesting they have little influence on prediction outcomes and explaining their consistently low modification frequencies.
\end{comment}



\begin{table}[h!]
\centering
\begin{tabular}{|l|l|c|c|c|}
\hline
\textbf{Feature} & \textbf{Factual Mode (\%)} & \textbf{CF Mode \%} & \textbf{$\delta_j$} \\
\hline
%Age band of driver & 31--50 (40.00\%) & xxx & 40.00\% & 0.00 \\
%Sex of driver & Male (100.00\%) & xx & 100.00\% & 0.00 \\
\textit{Driving experience} & Above 10yr (100.00\%) & 58.00\% & -0.42 \\
\hline
\textit{Types of Junction} & Crossing (100.00\%) & 56.00\% & -0.44 \\
\hline
\textit{Road surface type} & Asphalt roads (100.00\%) & 88.00\% & -0.12 \\
\hline
\textit{Light conditions} & Darkness -- lights lit (80.00\%) & 48.00\% & -0.40 \\
\hline
\textit{Weather conditions} & Normal (100.00\%) & 86.00\% & -0.14 \\
\hline
\textit{Type of collision} & Vehicle with vehicle collision (100.00\%) & 50.00\% & -0.50 \\
\hline
\textit{Vehicle movement} & Turnover (60.00\%) & 14.00\% & -0.77 \\
\hline
\textit{Pedestrian movement} & Not a Pedestrian (100.00\%) & 70.00\% & -0.30 \\
\hline
\textit{Cause of accident} & No distancing (40.00\%) & 36.00\% & -0.10 \\
\hline
\end{tabular}
\caption{Comparison of the most frequent (mode) feature categories for the factual and counterfactual samples of Region $1$. Factual Mode: Refers to the most frequent category for each feature in the original factual instances. Mode $\%$: Represents the proportion of factuals in that region with that categorical value. The $\%$ indicates the percentage of the factual mode in the counterfactual instances. CF Mode $\%$ presents the proportion of counterfactual feature values populated by the factual mode. $\delta_j$: Relative change rate from equation. Age and sex driver features are excluded since they were considered immutable.
}
\label{tab:mode_comparison}
\end{table}

\begin{comment}
\begin{table}[htbp]
\centering

\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|r|}
\hline
\textbf{Feature} & \textbf{Original Mode} & \textbf{Mode \%} & \textbf{Original Mode \% in CF  } &\delta_j \\
\hline

Driving experience      & Below 1yr                    & 66.67\%   & 55.00\%      &-0.175\\
\hline
Types of Junction      & Crossing                     & 83.33\%   & 60.00\%   &-0.28 \\
\hline
Road surface type       & Asphalt roads                & 100.00\%  & 100.00\%   &0\\
\hline
Light conditions        & Darkness - lights lit        & 100.00\%  & 85.00\%   &-0.15 \\
\hline
Weather conditions      & Normal                       & 100.00\%  & 98.33\%    &-0.017 \\
\hline
Type of collision      & Vehicle with vehicle collision & 100.00\% & 45.00\%  &-0.55\\
\hline
Vehicle movement        & Going straight               & 100.00\%  & 68.33\%   &-0.317\\
\hline
Pedestrian movement     & Not a Pedestrian             & 50.00\%   & 46.67\%     &-0.067 \\
\hline
Cause of accident      & No priority to pedestrian    & 50.00\%   & 41.67\%   &-0.167 \\
\hline

\end{tabular}%
}
\caption{Comparison of Mode Categories and Percentages in Original and Counterfactual Samples of Region $1$. Original Mode: Refers to the most frequent category for each feature in the original instances. Mode $\%$: Represents the percentage of the Original Mode. Original Mode $\%$ in CF: Indicates the percentage of the Original Mode in the counterfactual instances. $\delta_j$: Relative change rate from equation}
\label{tab:mode_comparison}
\end{table}
\end{comment}
\begin{comment}
\section{Mode}
The original factual samples from Region $1$ are compared with their generated counterfactual samples, focusing on the proportion of the mode for each feature.
\begin{table}[htbp]
\centering

\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|r|}
\hline
\textbf{Feature} & \textbf{Original Mode} & \textbf{Mode \%} & \textbf{Original Mode \% in CF  } &\delta_j \\
\hline

Driving experience      & Below 1yr                    & 66.67\%   & 55.00\%      &-0.175\\
\hline
Types of Junction      & Crossing                     & 83.33\%   & 60.00\%   &-0.28 \\
\hline
Road surface type       & Asphalt roads                & 100.00\%  & 100.00\%   &0\\
\hline
Light conditions        & Darkness - lights lit        & 100.00\%  & 85.00\%   &-0.15 \\
\hline
Weather conditions      & Normal                       & 100.00\%  & 98.33\%    &-0.017 \\
\hline
Type of collision      & Vehicle with vehicle collision & 100.00\% & 45.00\%  &-0.55\\
\hline
Vehicle movement        & Going straight               & 100.00\%  & 68.33\%   &-0.317\\
\hline
Pedestrian movement     & Not a Pedestrian             & 50.00\%   & 46.67\%     &-0.067 \\
\hline
Cause of accident      & No priority to pedestrian    & 50.00\%   & 41.67\%   &-0.167 \\
\hline

\end{tabular}%
}
\caption{Comparison of Mode Categories and Percentages in Original and Counterfactual Samples of Region $1$. Original Mode: Refers to the most frequent category for each feature in the original instances. Mode $\%$: Represents the percentage of the Original Mode. Original Mode $\%$ in CF: Indicates the percentage of the Original Mode in the counterfactual instances. $\delta_j$: Relative change rate from equation}
\label{tab:mode_comparison}
\end{table}
The table \ref{tab:mode_comparison} shows that the mode for each feature in the original data still holds the highest proportion in the counterfactual samples, although the overall percentages show a slight decline, meaning that all $\delta_j$ is negative or zero.
Among them, $Type\ of\ collision$ has a $\delta_j$ of $–0.55$, with an absolute value much higher than that of the other features. This indicates that during the counterfactual generation process, the proportion of the dominant category “Vehicle with vehicle collision” for $Type\ of\ collision$ experienced a significant change, suggesting that it may be the main factor driving the prediction from “severe” to “non-severe”, that make $Type\ of\ collision$ has high change frequency in Region $1$. 

Another feature in Region $1$ with a high change frequency is $Types\ of\ Junction$, whose $|\delta_j|$ is 0.28, which is still relatively high, but only half that of $Type\ of\ collision$. This demonstrates that the dominant category ‘Crossing’ for $Types\ of\ Junction$ is a relatively less important factor in causing the prediction to switch from “severe” to “non-severe”. 

In contrast, $Weather\ conditions$ and $Road\ surface\ type$ have $|\delta_j|$ values of $0.017$ and $0.00$, respectively, indicating that the dominant categories for these two features have little to no impact on the prediction change, which is why these two features have the lowest change frequencies.
\end{comment}
\subsection{Comparing Regional and Global Feature Change Frequency}


\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.47\textwidth}
    \centering
    \includegraphics[height=0.25\textheight]{SoGood_Workshop_Submission/figures/correlation_Global vs Region 1_ driving experience >10years (Pearson r = 0.45).pdf}
    \caption{Region 1: \textit{Driving experience} >10
years, r = 0.45}
    \label{fig:re1}
  \end{subfigure}%
  \hspace{0.5cm}
  \begin{subfigure}[t]{0.47\textwidth}
    \centering
    \includegraphics[height=0.25\textheight]{SoGood_Workshop_Submission/figures/correlation_Global vs Region 2 driving experience <1 year (Pearson r = 0.47).pdf}
    \caption{Region 2: \textit{Driving experience} <1 
year, r = 0.47}
    \label{fig:re2}
  \end{subfigure}

  \vspace{0.1cm}
  
  \begin{subfigure}[t]{0.47\textwidth}
    \centering
    \includegraphics[height=0.25\textheight]{SoGood_Workshop_Submission/figures/correlation_Global vs Region 3 Weather = rainy (Pearson r = 0.33).pdf}
    \caption{Region 3: \textit{Weather conditions} =
"rainy",  r = 0.33}
    \label{fig:re3}
  \end{subfigure}%
  \hspace{0.5cm}
  \begin{subfigure}[t]{0.47\textwidth}
    \centering
    \includegraphics[height=0.25\textheight]{SoGood_Workshop_Submission/figures/correlation_Global vs Region 4_ Weather = Normal (Pearson r = 0.66).pdf}
    \caption{Region 4: \textit{Weather conditions} =
"normal",  r = 0.66}
    \label{fig:re4}
  \end{subfigure}
  
\caption{Plotting the global feature change frequency values against those for each region. Pearson correlation coefficients ("r") are presented for each.}
\label{fig:overallre}
\end{figure}

\begin{comment}
As shown in the figure \ref{fig:overallre}, the horizontal axis represents the Global Frequency, and the vertical axis represents the Local Frequency. By comparing the frequency values of each feature at the global and local levels within each region, the Pearson correlation coefficient ($r$ value) for each region is computed.
From figure \ref{fig:re1}, for Region 1, the correlation coefficient with the global data is $r$ = 0.31. In the global dataset, the change frequencies of $Driving\ experience$ and $Cause\ of\ accident$ are relatively high, whereas in the local data these two exhibit relatively lower change frequencies, showing a ``high in global, low in local" pattern. In contrast, although the change frequencies of $Types\ of\ Junction$ and $Type\ of\ collision$ are not particularly prominent in the global data, they increase significantly in the local data, displaying a ``high in local, low in global" trend; meanwhile, $Road\ surface\ type$, $Light\ conditions$, $Weather\ conditions$, and $Pedestrian\ movement$ remain low in both the global and local datasets. This inconsistency in the ordering of change frequencies for some features results in only moderate overall agreement for Region 1, leading to an $r$ value of 0.31.

As shown in figure \ref{fig:re2}, for Region 2, the correlation coefficient with the global data is $r$ = 0.25. The change frequencies of $Driving\ experience$ and $Cause\ of\ accident$ are high in the global data, but they decrease in the local data, exhibiting a ``high globally, low locally" pattern. Meanwhile, the change frequencies of $Types\ of\ Junction$ and $Type\ of\ collision$ are significantly higher locally, displaying a ``high locally, low globally" trend. $Road\ surface\ type$, $Light\ conditions$, and $Weather\ conditions$ remain at low levels in both the global and local data. Since the ranking of change frequencies for some features does not fully correspond between the local and global data, the overall consistency of the ranking in Region 2 is weak, with an $r$ value of only 0.25.

As shown in the figure \ref{fig:re3}. In Region 3, the Pearson correlation coefficient between the local and global change frequencies is $r$ = 0.40. The variation frequency of $Types\ of\ Junction$ in the local region is significantly higher than in the global data, exhibiting a ``local high, global low" pattern, whereas $Driving\ experience$, which has a high variation frequency globally, is reduced locally, demonstrating a ``global high, local low" trend. In addition, both $Road\ surface\ type$ and $Weather\ conditions$ maintain low variation frequencies in both global and local data. Overall, the ranking of feature variation frequencies in Region 3 aligns well with the global baseline, which explains its relatively high $r$ value of 0.40.

As shown in the figure \ref{fig:re4}. In Region 4, the Pearson correlation coefficient between the local and global change frequencies is $r$ = 0.36, and the situation is similar to that in Region 3. $Driving\ experience$ originally exhibits a high change frequency at the global level, but its frequency decreases in the local data, forming a ``global high, local low" pattern. In contrast, $Types\ of\ Junction$ and $Light\ conditions$ increase from relatively low levels globally to much higher levels locally, displaying a ``local high, global low" pattern. $Road\ surface\ type$ and $Weather\ conditions$ remain low in both global and local settings, and $Type\ of\ collision$ is essentially unchanged between the two. This shift in the ordering of change frequencies for some features results in an overall moderate consistency in Region 4, with an $r$ value of 0.36.

As shown in the figure \ref{fig:re5}, The Pearson correlation coefficient between the local and global change frequencies of Region 5 is $r$ = -0.21, indicating a completely different distribution. In this region, the change frequency of $Driving\ experience$, which is high globally, is significantly reduced in the local data, exhibiting a ``globally high, locally low" pattern. In contrast, $Types\ of\ Junction$, $Road\ surface\ type$, $Weather\ conditions$, $Vehicle\ movement$, and $Pedestrian\ movement$, which have relatively low change frequencies in the global data, increase in the local data, showing a ``locally high, globally low" pattern. This complete reversal in overall ranking results in the ordering of feature change frequencies in Region 5 being almost entirely opposite to the global benchmark, leading to a negative $r$ value of -0.21.

Finally, as shown in the figure \ref{fig:re6}, Region 6 has a correlation of $r$ = 0.2$2$ with the global data. In this region, the change frequency for $Types\ of\ Junctio$n clearly increases locally, exhibiting a ``locally high, globally low" trend; whereas the change frequency for $Cause\ of\ acciden$t drops from a high global level to a lower local level, representing a ``globally high, locally low" pattern. In addition, $Light\ conditions$, $Weather\ conditions$, $Vehicle\ movement$, and $Pedestrian\ movement$ are relatively low in both global and local contexts. Due to the significant changes in some key features in the local data, the overall consistency of Region 6 is weakened, resulting in an $r$ value of only 0.2$2$.
\end{comment}


Figure \ref{fig:overallre} presents a comparison of global and regional feature change frequency. As outlined in Figure \ref{fig:egr}, this provides a means to assess alignment between global and local feature importance.

Both of the regions focused on the amount of driving experience, Regions 1 and 2 (Figure \ref{fig:re1} and \ref{fig:re2}) show a moderate correlation between global and regional feature change frequency: $r$ = 0.45 and $r$ = 0.47 respectively. The low regional and global impact of \textit{road surface type} (red circle on the plots) on accident severity is consistent between both the experienced and inexperienced drivers. Other than that, there are variations in which features align well with the global feature change frequency (near to the red dashed diagonal line) and those which stray from it. \textit{Vehicle movement} for Region 1, the experienced drivers, has a particularly high importance for this specific region and a modest global importance. For Region 1 most of the features are more important in this region than globally (above the dashed line), indicating that this group of accidents is quite different to the wider data set of road accident events.

The two regions which were chosen for differing \textit{Weather conditions}, Figures \ref{fig:re3} and \ref{fig:re4}, higher levels of contrast are observed. Region 3, chosen for its grouping of incidents occurring with "rainy" conditions had the lowest correlation between global and regional feature changes with $r$ = 0.33. This was largely driven by the strong regional effect of the weather conditions feature itself. By contrast, Region 4, for accidents with "normal" \textit{Weather conditions} had the strongest correlation ($r$ = 0.66) and features that most resembled a y = x relationship. Therefore suggesting that of the four presented regions the accidents represented by Region 4 are themselves the most similar to the average of all accidents in the dataset.

The presented regions show only weak to moderate alignment between global and regional feature change frequencies, indicating that counterfactual explanations are region-specific and influenced by local feature distributions. Suggesting that explanations based on global patterns may not generalize well across all data subsets. These results underscore the importance of analyzing counterfactual behavior at both global and localized levels for more accurate and context-sensitive interpretability. Furthermore, this form of analysis could provide a complementary means to assess how similar a localised group of instances are to the wider data set, and to highlight similarities and differences to feature importances across a data set.






==> chapters/appendices/app0A.tex <==
%
% file: localoperator.tex
% author: Victor Brena
% description: Briefly describes properties of the local operator.
%

\chapter{Appendix A}
\label{app:app01}

Begins an appendix









\

==> chapters/chapter01/chap01.tex <==
%
% File: chap01.tex
% Author: Victor F. Brena-Medina
% Description: Introduction chapter where the biology goes.
%
\chapter{Introduction}
\label{chap:intro}
In recent years, machine learning models, particularly deep neural networks and complex ensemble methods, have achieved state of the art performance on a wide range of tasks. 

However, their internal decision processes remain opaque, earning them the label of “black box” models. Because users and stakeholders cannot directly inspect how inputs are transformed into outputs, these models raise concerns about trust, accountability, and safety, especially in critical applications such as healthcare, finance, and traffic safety.\cite{guidotti2024counterfactual}.

Explainable AI (XAI) aims to address this challenge by providing tools that illuminate model behavior. Among these tools, counterfactual explanations have proven especially intuitive and practical. A counterfactual explanation explores what if scenarios by asking how targeted changes to input features would alter the model’s prediction\cite{wachter2017counterfactual}. Formally, given an instance $X$ with model output $a(X)$, a counterfactual $X'$ satisfies $a(X')\neq a(X)$ while minimizing the difference $||X'-X||$. This approach reveals the minimal adjustments needed to change the decision.

Counterfactual explanations may be chosen to exhibit properties such as validity, proximity, sparsity, diversity, actionability and causality. These properties enable them to generate clear explanations and provide practical recommendations. They have been applied in fields ranging from medical diagnosis\cite{richens2020improving} to financial decision making\cite{cornacchia2023auditing}, demonstrating their ability to uncover implicit causal relationships and to guide individual choices.

In traffic safety, reducing accident severity is critical. Traffic collisions result from interactions among factors such as vehicle speed, weather and lighting conditions, road design, and driver characteristics. Prediction models alone do not indicate how to intervene most effectively. Through counterfactual analysis on an accident severity predictor, one can simulate alternative scenarios such as “How would severity change if speed were reduced by 10 $km/h$?” or “What if the road had been dry?” and quantify each factor’s impact on predicted severity. Such insights can inform safety interventions, driver advisories, and infrastructure improvements.

This report introduces a global and local counterfactual explanation framework for a random forest classifier trained on a dataset of 12,316 samples with 12 features, collected from manual records of road traffic accidents by the Addis Ababa Sub‑city, the capital city of Ethiopia in East Africa, during 2017–2020. From a global perspective, overall feature importance is established by measuring how often each feature must be changed to flip a prediction of accident severity  from “severe” to “non‑severe”. From a local perspective, multiple counterfactuals are generated for each individual case and its neighborhood of similar instances to uncover the specific factors driving severity. The Pearson correlation coefficient is used to quantify the agreement between global and local feature importance, explanation sparsity is evaluated, and shifts in each feature’s dominant category are examined. The results show that counterfactual explanations both elucidate the model’s decision logic and provide actionable insights for reducing traffic accident severity.
%=========================================================

==> chapters/chapter02/chap02.tex <==
\chapter{Literature review}
\label{chap:Liter}
\section{Features  Affecting accident severity}
Lighting conditions have a significant impact on accident severity. In a completely dark environment with no street lighting at night, the risk of fatalities and serious injuries is $33$ times higher than during the day, indicating that insufficient lighting is a key factor in exacerbating accident severity\cite{yannis2013effect}. The effect of driving experience on accident severity presents a complex duality. Although experienced drivers possess stronger vehicle control skills, their optimism bias and tendency to attribute accidents to external factors—such as road defects, weather, or pedestrians—rather than their own responsibility reduce their active hazard-avoidance awareness, making them more likely to cause severe accidents in complex traffic conditions due to overconfidence. In contrast, novice drivers, despite potentially overestimating their ability to cope because of cognitive limitations, tend to have accidents caused by misjudgments, resulting in relatively lower severity\cite{kouabenan2002occupation}. \par

Junction type also plays an important role in accident severity. Roundabouts and small roundabouts, due to enforced speed reductions and the design of a single conflict point, have the lowest fatality and serious injury rates; however, T-shaped/misaligned intersections and crossroads, because of obstructed sightlines and multi-directional conflicts, exhibit a serious injury risk of up to $75.9\%$ at night, making them the most dangerous types\cite{wu2019crash}. Multiple intersections increase the risk of vehicle mispositioning due to their complex lane configurations, while “other types” of intersections exhibit a highly variable distribution in accident severity due to mixed traffic flows\cite{wu2019crash}.\par

Regarding pavement physical characteristics, when the International Roughness Index (IRI) exceeds $3.2 m/km$, the accident rate increases by 1.5 times, especially on rainy nights when rough pavement decreases vehicle handling stability,r oads with rut depths over 23.5mm are prone to water accumulation, leading to aquaplaning. Thereby increasing accident probability by $40\%$; and in slippery conditions. Inadequate skid resistance accident risk to surge by $68\%$\cite{mkwata2022effect}. \par

Furthermore, collision type has a significant impact on accident severity, with frontal/side collisions being more likely to lead to severe outcomes compared to rear-end or collision with obstacles\cite{eboli2020factors}. Weather conditions also influence accident severity in England and Wales. Accidents in rainy weather are significantly less severe than those on clear days, possibly because drivers reduce speed and drive more cautiously in the rain, although slippery roads might also lead to more minor collisions, thereby lowering the overall severity ratio. In contrast, the severity of accidents in fog shows regional differences; drivers in areas where fog is common are more familiar with the roads and thus face lower risks, whereas in regions where fog is rare, the consequences of accidents tend to be more severe. The impact of strong winds, meanwhile, is inconsistent, with some counties experiencing increased accident severity and others a decrease, likely due to variations in drivers’ experience in handling sudden gusts\cite{edwards1998relationship}.
\section{Counterfactuals}
Due to the lack of transparency in black-box models such as deep neural networks, people still lack confidence in the output of AI systems\cite{guidotti2018survey}\cite{miller2019explanation}, as they cannot understand the reasoning behind the model’s decisions \cite{freitas2014comprehensible}. Counterfactuals can address this by demonstrating how changing certain input features leads to changes in the output\cite{wachter2017counterfactual}. For example, if a person applies for a loan from a bank, and the AI system of the bank informs that this person are not eligible for the loan and did not provide any further insight into why the person could not get this loan, this person would not know what changes to make to qualify for it. A counterfactual, however, would provide an answer like, `If you increase your annual income from £12,000 to £15,000, you will qualify for the loan.' This kind of response contrasts with the real situation, embodying the principle of “if $X$ had not happened, $Y$ would not have occurred,” which is the fundamental idea of counterfactuals, meaning that due to changes in certain features, the outcome is opposite to the fact\cite{mothilal2020explaining}. Suppose a classifier $a$ outputs decision $Y=a(X)$ for instance $X$, then a counterfactual explanation consists of an instance $X^'$, such that classifier $a$ outputs a decision for $X^'$ that differs from $Y$,  $a(X')\neq Y$ \cite{guidotti2024counterfactual}.

Counterfactual explanations have several desirable properties, including validity, minimality, similarity, diversity, actionability, and causality:

Validity: A counterfactual $X'$ is valid if and only if it changes the original input result, $a(X^')$$\neq a(X)$\cite{guidotti2024counterfactual,mothilal2020explaining,molnar2020interpretable,verma2024counterfactual}.

Sparsity: Sparsity means that when generating a counterfactual, the number of features that need to be changed should be minimized to ensure the explanation is concise and clear, meaning that there should not exist another counterfactual instance $X''$ such that $|\delta_{X,X''}| < |\delta_{X,X'}|$, where $|\delta_{X,X'}|$ represents the number or magnitude of feature changes from the original factual instance $X$ to the counterfactual instance $X'$. For example, a loan application model rejects an applicant's loan request. If the counterfactual explanation suggests that the applicant only needs to increase their annual income from £12,000 to £15,000  to get approved, then this explanation is sparse. In contrast, if the counterfactual explanation suggests changing multiple features such as income, age, and place of residence, it would lose minimality, making the suggestions complex and difficult to execute\cite{guidotti2024counterfactual,verma2024counterfactual}.

Proximity: The distance between counterfactual instance $X'$ and original factual instance $X$ in feature space should be as small as possible. The generated counterfactual instance should be a slight adjustment to the original instance, making these changes feasible in practice. This should satisfy $d(X, X') < \epsilon$, where $d(X, X')$ is the distance between $X$ and $X'$ in feature space, and $\epsilon$ is a predefined maximum distance threshold to limit the deviation between the counterfactual and the original instance\cite{guidotti2024counterfactual,mothilal2020explaining,verma2024counterfactual}.

Diversity: Counterfactual explanations should not focus on only one way of changing the original input to alter the model’s output, but instead provide multiple distinct paths. Each path represents a possible change to achieve the desired result. Given a set of counterfactuals \{$X'_0, X'_1, ...$\}, diversity should be ensured by maximizing $d(X'_0, X'_1)$, where $d(X'_0, X'_1)$ is the distance function used to measure the difference between two counterfactual instances\cite{guidotti2024counterfactual,mothilal2020explaining,karimi2020model}.

Actionability: The feature changes in the counterfactual instance should be controllable and feasible for the user. In the aforementioned loan example, if the counterfactual instance is``If you were ten years younger, you could get the loan'' or ``If you increase your income by 1000 times, you could get the loan" the former is clearly impossible since age is an uncontrollable feature, and the latter is also extremely difficult to achieve under normal circumstances\cite{guidotti2024counterfactual,verma2024counterfactual}.

Causality: The features changed in the generated counterfactual instance should have a substantial causal impact on the model's decision, rather than being irrelevant or secondary features. Methods such as Bayesian networks and causal graphs can be used in advance to exclude features with weak causal relationships\cite{guidotti2024counterfactual,verma2024counterfactual}.\par
Global explanation and local explanation are two core analytical methods. Global explanation focuses on the behavioral patterns of the model across the entire dataset by analyzing the overall impact of features on predictions, such as through SHAP's global feature importance or partial dependence plots that reveal the model’s generalization logic. In contrast, local explanation concentrates on the prediction result of a single instance, using sensitivity analysis or counterfactual generation to explain the causal relationship between specific inputs and outputs. The core difference between the two lies in their scope of analysis: global methods provide a macroscopic insight into the overall behavior of the model, while local methods uncover the microscopic mechanisms behind individual decisions\cite{kommiya2021towards,mishra2021survey}.\par
Based on this, two computation methods for counterfactual feature importance (CFI), one called “Greedy CFI” based on a greedy strategy and the other “CounterShapley CFI” based on Shapley values have been proposed to quantify the impact of feature modifications on model predictions, accompanied by visualization tools such as Greedy Chart, CounterShapley Chart, and Constellation Chart to enhance the intuitiveness of the explanations\cite{meulemeester2023calculating}. However, the effectiveness of these methods depends on the sparsity and diversity of the generated counterfactuals. Further research indicates that the explanations must satisfy Validity, yet traditional feature attribution methods such as LIME and SHAP often fail to meet these two standards; for example, in the Adult Income dataset, modifying features outside the top three more readily generates effective counterfactuals, and there is a significant difference in the feature importance ranking between counterfactual methods and feature attribution methods\cite{kommiya2021towards}. Moreover, the robustness of explanation methods faces multiple challenges: input perturbations, model updates, and hyperparameter sensitivity. In response, proposed improvements include data manifold projection, stability regularization, and the Counterfactual Stability metric\cite{mishra2021survey}.

\section{AI in traffic accident}
The use of artificial intelligence techniques to directly predict or analyse traffic accident severity has become an important research direction in the field of traffic safety. By using machine learning and deep learning models, effective features can be extracted from multidimensional traffic data to predict and explain accident severity. The problem of traffic accident prediction was explored using models such as Random Forest and it was pointed out that factors such as speed, weather, and road conditions have a significant influence in prediction\cite{siswanto2023artificial}. The prediction results of models such as gradient boosting were interpreted using the SHAP method, and the role of key variables such as speeding and road category on accident fatality was clarified\cite{panda2023predicting}.\par
There is also an accident severity prediction model based on artificial neural networks, which constructs a multi-layer feed-forward neural network, which iteratively optimises the weights of the layers within the network by employing a back-propagation algorithm in order to minimise the error between the predicted output and the true accident severity category. During the model training process, the generalisation ability of the model across different datasets is ensured by normalising preprocessing and cross-validation of the input features\cite{hamdan2023traffic}. In addition, research using Transformer and various deep learning architectures in combination with explanatory AI techniques has further improved the transparency and reliability of the prediction models by quantitatively analysing the contribution of multiple features\cite{aboulola2024automated}. \par
From a risk analysis perspective, XGBoost, Random Forest and Deep Neural Networks were integrated and SHAP values were used to reveal the impact of driving behaviour and environmental factors on injury severity, providing a more intuitive basis for decision-making\cite{abdulrashid2024explainable}.\par

Compared to other AI methods, the counterfactual approach has the following advantages in traffic accident prediction; firstly, it can provide explicit and actionable suggestions to transform model-predicted severe accidents into non-severe ones; secondly, through multi-instance counterfactual interpretation, the approach is able to generate global improvement proposals for a group of accident cases simultaneously, instead of limiting itself to a single case, thus better capturing group characteristics ; moreover, the method improves the interpretability of the black-box model by ensuring the feasibility and cost-effectiveness of the recommendations while minimising attribute changes\cite{artelt2021application}.

==> chapters/chapter03/chap03.tex <==
\chapter{Methodology}
\label{chap:Method}
\section{Dataset and Model Training}
Before generating counterfactual explanations using DiCE, it is first necessary to train a predictive model. Before model training, the data is preprocessed and divided into an $80\%$ training set and a $20\%$ test set. The dataset contains $12,316$ samples and $12$ features \eqref{tab:ft}, collected from traffic accident records of the Addis Ababa Sub-city Police Department during the years 2017 to 2020. Random forest classifier was chosen as the base algorithm, because as an ensemble learning method, random forest effectively captures complex relationships among features by constructing multiple decision trees and using voting to make stable, robust predictions. Random forest not only performs well in multi-class classification tasks, but its ensemble structure also helps reduce the risk of overfitting and effectively handle noise and outliers in the data, leading to relatively stable decision logic. Based on this model, DiCE is applied to analyze the decision boundaries and generate counterfactual instances. These instances, created by making minimal adjustments to the input features, demonstrate which slight changes can lead to a different prediction, thereby helping to explain the model’s decision-making process and identify the key features driving the prediction.\par
\section{Feature Encoding and Preprocessing}
$Accident\ severity$ is the target variable $(y)$ of the model in this project, different from other features in the dataset that serve as input variables $(X)$. $Accident\ severity$ represents the outcome of a traffic accident, such as minor or severe. It is a dependent variable determined by the changes in other input features, and its main role is to help predict the severity of the accident. And table \eqref{tab:ft} shows input features:\\
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    Features & Number of Categories & Nominal/Ordinal \\
    \hline
         Age-band of driver & 5 & Ordinal \\
    \hline
         Sex of driver & 3 & Nominal \\
    \hline             
         Driving experience & 7 & Ordinal \\
    \hline             
         Types of Junction & 8 & Nominal \\
    \hline             
         Road surface type & 6 & Nominal \\
    \hline             
         Light conditions & 4 & Nominal \\
    \hline             
         Weather conditions & 9 & Nominal \\
    \hline             
         Type of collision & 10 & Nominal \\
    \hline             
         Vehicle movement & 13 & Nominal \\
    \hline             
         Pedestrian movement & 9 & Nominal \\
    \hline
         Cause of accident & 20 & Nominal \\
    \hline                  
    \end{tabular}
    \caption{Summary of the 11 input features, showing for each the number of categories and whether the feature is ordered.}
    \label{tab:ft}
\end{table}


To adhere to the actionability of counterfactuals, $Age-band\ of\ driver$ and $Sex\ of\ dirver$ were set as immutable features. This means that these features were fixed and not allowed to change during the counterfactual generation process, as they are factors that cannot be altered in a real driving scenario. \par
 

Both the random forest model and DiCE rely on numerical input data for their internal computations. Although random forest model can theoretically handle categorical variables, in practice non numerical data are often required to be converted into numerical form for distance calculations and node splitting. Similarly, DiCE needs to compute distances and similarities in feature space when generating counterfactual explanations; if features remain in text form such mathematical operations cannot be directly performed. Therefore, all categorical variables must be encoded by assigning a unique numerical value to each category, thus converting textual data that originally cannot be used in mathematical computations into numbers that can participate in these operations. This approach not only facilitates the statistical analysis of the distribution, frequency, and correlations of each category with other variables, but also ensures consistency of the data during model training and counterfactual generation. By preserving this mapping, numerical codes can be reverse-converted back into the original textual labels when interpreting counterfactual explanation results, thereby ensuring that the final explanations remain readable.\par

\section{Counterfactual Generation with DiCE}
After randomly selecting several samples from the entire test set, multiple counterfactual instances are generated for each selected sample using DiCE, with the goal of changing the model's prediction from ``severe" to ``non-severe."

\section{Performance Evaluation}
The F1 score equation\eqref{eq:4} and accuracy equation\eqref{eq:5} were used to evaluate the performance of the Random Forest model. Accuracy measures the proportion of correct predictions among all predictions made by the model. It presents the overall correctness of the model, but it can be misleading for imbalanced datasets, as it may mask incorrect predictions for certain classes. The F1 score is the harmonic mean of precision and recall, and is particularly useful in cases of class imbalance. The F1 score provides a more balanced assessment of model performance because it takes into account both false positives and false negatives, making it an important metric for assessing model reliability when dealing with imbalanced class distributions.\par
\begin{equation}\label{eq:4}
    F1 = 2 \times \frac{Precision\times Recall}{Precision + Recall}
\end{equation}
\begin{equation}
    Precision = \frac{TP}{TP+FP}
\end{equation}
\begin{equation}
    Recall = \frac{TP}{TP+FN}
\end{equation}
\begin{equation}\label{eq:5}
    Accuracy = \frac{TP+TN}{TP+TN+FP+FN}
\end{equation}
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
        Symbol	 & Name & Description \\
        \hline
        TP & True Positives& The number of correct positive predictions by the model\\
        \hline
        TN& True Negatives&The number of correct negative predictions by the model\\
        \hline
        FP&False Positives&The number of incorrect positive predictions by the model\\
        \hline
        FN&False Negatives&The number of incorrect negative predictions by the model\\
        \hline
    \end{tabular}
    \caption{The names and explanations of the variables in the formulas for F1 score and accuracy }
    \label{tab:my_label}
\end{table}


\section{Feature Change Frequency}
Change frequency can serve as a key metric for evaluating the importance of features in counterfactual explanations. It is defined as the proportion of times a feature is changed during the generation of counterfactual instances. The basic idea is that if a feature is frequently modified in counterfactual instances, it may play an important role in altering the model’s prediction; conversely, if a feature is seldom changed, it may be critical in maintaining the original prediction. This frequency metric can be applied to both global and local explanations.
\subsection{Global Feature Change Frequency}

In the global explanation, the overall modification frequency of each feature is determined by statistically analyzing all the counterfactual instances generated for every sample in the dataset, thereby identifying the key features that consistently drive prediction changes across the entire dataset. The global modification frequency $F_j$ for feature $X_j$ is calculated using the following formula:
\begin{equation}
    F_{j}=\frac{1}{N \times n_{C F}} \sum_{i=1}^{N} \sum_{k=1}^{n_{C F}} I\left(X_{j}(i, k) \neq X_{j}(i, \text { orig })\right)
\end{equation}

Suppose there are $N$ samples, and for each sample,$n_{CF}$ counterfactuals are generated. For the $i$th sample, let the original value of feature $X_j$ be denoted as $X_j(i,orig)$ , and let the value in the $k$th counterfactual instance of the $i$th sample be denoted as $X_j(i,k)$. By comparing $X_j(i,k)$ with $X_j(i,orig)$, using an indicator function $I(\cdot)$ that returns $1$ if the values differ and $0$ otherwise \eqref{eq:6}, it is recorded whether the feature changes in each counterfactual instance. The inner summation $\sum_{k=1}^{n_{C F}}$ iterates over all counterfactual instances for each sample and the outer summation $\sum_{i=1}^{N}$ iterates over all samples.
\begin{equation}\label{eq:6}
    I\left(X_{j}(i, k) \neq X_{j}(i, \text { orig })\right)=\left\{\begin{array}{ll}
1, & \text { if } X_{j}(i, k) \neq X_{j}(i, \text { orig })  \\
0, & \text { otherwise }
\end{array}\right.
\end{equation}

\subsection{Local Feature Change Frequency}

In local explanations, the change frequency of each feature is calculated for an individual sample's counterfactual instances, revealing how minor adjustments in that sample affect the prediction outcome.

$n_{CF}$ counterfactual instances are generated for a given sample and the modification frequency for each feature is computed as a measure of its influence in that specific instance. Let $X_j(orig)$ denote the original value of feature $X_j$ of the target sample, and $X_j(k)$ denote the value of $X_j$ in the $k$th counterfactual instance. The local modification frequency $f^{local}_j$ is defined as follows:
\begin{equation}
    f_j^{local}=\frac{1}{n_{CF}}\sum_{k=1}^{n_{CF}}I\left(X_{j}(k) \neq X_{j}(\text { orig })\right)
\end{equation}
where the indicator function $I(\cdot)$ is defined by formula \eqref{eq:6}
\subsection{Region and Neighbors of Single Local Sample }
Neighbor analysis is incorporated to construct a target region composed of the most similar samples in the feature space, referred to as ``neighbors." Neighbors are other samples with the highest similarity to a given query sample in the encoded and normalized feature space. All categorical variables are encoded and normalized to ensure comparability, and Hamming distance is employed as the metric, which is suitable for encoded categorical data to quantify the similarity between samples. Subsequently, a nearest neighbor algorithm is used to identify the samples most similar to the given query sample. Hamming distance is defined as:
\begin{equation}
    d_h(x,y)=\sum_{j=1}^{m}I(x_j\neq y_j)
\end{equation}

Within this target region, the modification frequency of each feature is computed from the counterfactual instances generated from these neighbors, and the average and standard deviation of these local modification frequencies are further calculated.
\begin{equation}
    \overline{f_j^{re}}=\frac{1}{N}\sum_{i=1}^{N}f_j^{local}(i)
\end{equation}
$\overline{f_j^{re}}$ represents the mean local change frequency of feature $j$ across all samples, $N$  denotes the total number of samples considered, and $f_j^{local}(i)$ represents the local change frequency of feature $j$ for the $i$th sample in this region.

\begin{equation}
    \sigma_{f_j^{local}}=\sqrt{\frac{1}{N}\sum_{i=1}^{N}(f_j^{local}(i)-\overline{f_j^{re}})^2}
\end{equation}
$\sigma_{f_j^{local}}$ denotes the standard deviation of the local change frequency of feature $j$, which measures the variability of this frequency across different samples.
\section{Correlation Analysis of Local and Global Change Frequencies}
By correlating the average local change frequency for each feature in a given region $\overline{f_j^{re}}$ with its global change frequency $F_j$, the alignment of local counterfactual explanations with overall trends is evaluated. The Pearson correlation coefficient (PCC) is calculated as follows:
\begin{equation}
    r=\frac{\sum_{j=1}^{m}(\overline{f_j^{region}}-\mu_{re})(F_j-\mu_{g})}{\sqrt{\sum_{j=1}^{m}(\overline{f_j^{region}}-\mu_{re})^2}\sqrt{\sum_{j=1}^{m}(F_j-\mu_{g})^2}}
\end{equation}
In this formula, $\mu_{re}=\frac{1}{m}\sum_{j=1}^{m}\overline{f^{re}_j}$ represents the mean of the average local change frequencies for all features in the region, while $\mu_{g}=\frac{1}{m}\sum_{j=1}^{m}F_j$ denotes the mean global change frequency across all features.

In the figure \ref{fig:egr}, the example points A, B, C, and D are solely used to illustrate the distribution of feature importance in both global and local contexts; their positions are provided merely for reference.

Point A represents data in the upper-left quadrant, where the feature exhibits low global importance but high local importance. This indicates that while the feature does not significantly impact the overall model predictions, it is very important for specific samples or groups of similar samples. 

Point B represents data in the lower-left quadrant, where the feature neither stands out on a global scale nor exhibits exceptional prominence locally, suggesting that its influence on model predictions remains low both overall and locally. 

Point C represents data in the upper-right quadrant, where the feature has high importance in both global and local dimensions, signifying that it plays a crucial role not only in the overall dataset but also within specific samples or neighborhoods. 

Point D represents data in the lower-right quadrant, where the feature shows high global importance but is not prominent locally, indicating that, although it has a significant impact on overall model predictions, its importance does not manifest in some individual samples or local regions. 

The figure also displays the reference line y = x, which represents the ideal state of perfect consistency between local and global feature importance, corresponding to a correlation coefficient r value of 1. Therefore, the distance of a data point from this line reflects the degree of consistency or deviation between its global and local importance.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{egr.png}
    \caption{Example points A, B, C, and D are for illustration only: A indicates low global but high local importance; B shows both are low; C indicates both are high; and D shows high global but low local importance. The distance of each point from the line y = x reflects the consistency or deviation between global and local importance.}
    \label{fig:egr}
\end{figure}
\section{Global Feature Modification Sparsity Analysis}
To evaluate the sparsity of the counterfactual explanations, in the global explanation stage, each counterfactual instance is compared with its corresponding original sample one by one using the indicator function \eqref{eq:6} to determine whether each feature has changed, and the number of changed features is calculated for each counterfactual instance. Then, the change counts for all counterfactual instances are aggregated to obtain the global distribution of feature changes.

\section{Local Main Characteristics}
To observe the distribution of each feature within a specific sample and its similar sample group, and to determine whether significant shifts occur during counterfactual generation, a mode statistics method is employed in the local analysis. Specifically, the most common category and its proportion are first calculated for each feature in the original data, revealing the primary distribution of that feature. Then, the same statistics are performed on the counterfactual data generated for the specific sample and its similar sample group, calculating the proportion of the category with the highest occurrence count in the counterfactual data while also recording the proportion of the mode from the original data as it appears in the counterfactual instances. By comparing the mode proportions of each feature in the original and counterfactual data, as well as the changes in the mode's proportion from the original data in the counterfactual instances, it becomes possible to directly observe whether significant adjustments have been made to certain features during the counterfactual generation process.

The relative change rate is defined as:
\begin{equation}\label{eq:rc}
    \delta_j=\frac{p_j^{cf}-p_j^{orig}}{p_j^{orig}}
\end{equation}
where $p_j^{orig}$ is the proportion of the most common category for feature $j$ in the original sample, and $p_j^{cf}$ This metric quantifies the percentage change in the proportion of that category during the counterfactual generation process and provides a standardized measure. If $\delta_j$ is positive, it indicates that the proportion of that category has increased in the counterfactual data; if negative, the proportion has decreased.

When $|\delta_j|$ is small, it indicates that the counterfactual generation process has little impact on the main distribution of that feature, demonstrating that the local explanation is relatively stable and consistent with respect to that feature. Conversely, when $|\delta_j|$ is large, it suggests that significant shifts occur in that feature during the counterfactual generation process, which may imply that the feature plays a more critical role in the local explanation.

==> chapters/chapter04/chap04.tex <==
\chapter{Result and Discussion}
\label{chap:RD}
\section{Model Performance Evaluation}
The F1 score of $0.78935$ demonstrates that the model achieves a good balance between precision and recall. According to the methodological definition of the F1 score, when severe accident samples are relatively scarce, the F1 score can more effectively capture the model’s ability to recognize the minority class. A score close to 0.79 indicates that the model has reached an appropriate compromise between preventing false positives and avoiding false negatives, thereby accurately identifying truly severe accident cases in practical applications.

An accuracy of $83.47\%$ reflects that the model is capable of correctly classifying the majority of samples overall. As noted in the methodology, although accuracy is an intuitive indicator of overall prediction correctness, it may obscure deficiencies in detecting the minority class when the data exhibits class imbalance. Therefore, even though the relatively high accuracy indicates that most predictions are correct, relying solely on this metric might not fully evaluate the model’s performance in capturing the critical minority of severe accidents. Taken together, the current scores show that the model not only maintains high overall prediction accuracy but also effectively identifies important minority classes in a complex and imbalanced data environment.

\section{Counterfactual Explanation}
For the randomly selected factual instance labeled “severe,” five counterfactual instances were generated, each configured to exhibit a “non severe” accident severity outcome. In each counterfactual, one or two features are modified, causing the accident severity to change to ``non-severe". Figure \ref{fig:tezheng} displays the feature modifications in these five counterfactual explanations.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{tezheng.png}
    \caption{Five generated counterfactuals for reducing accident severity from “severe” to “non-severe”.}
    \label{fig:tezheng}
\end{figure}
\section{Feature Change Frequency}
\subsection{Global Feature Change Frequency }
A total of $2000$ factual instances were selected, and for each instance, a counterfactual was generated to calculate the global feature change frequency.

In the figure \ref{fig:gl}, the horizontal axis represents the features, while the vertical axis shows the corresponding average change frequency ranging from $0$ to $1$. Specifically, the change frequency for $Cause\ of\ accident$ is $0.38$, the highest among all features; $Driving\ experience$ follows at $0.376$; $Type\ of\ collision$ is $0.26$; $Vehicle\ movement$ is $0.228$; $Weather\ conditions$ is $0.196$; $Types\ of\ Junction$ is $0.192$; $Light\ conditions$ is $0.164$; $Pedestrian\ movement$ is $0.148$; and $Road\ surface\ type$ is $0.136$. Table \ref{tab:feature_importance} presents the resulting importance ranking.
\begin{table}[htbp]
\centering
\begin{tabular}{|c|c|c|}

\hline
Rank & Feature              & Change Frequency \\
\hline

1    & Cause of accident   & 0.38           \\
\hline
2    &Driving experience    & 0.367            \\
\hline
3    &Type of collision    & 0.26           \\
\hline
4    & Vehicle movement    & 0.228            \\
\hline
5    & Weather conditions  & 0.196             \\
\hline
6    & Types of Junction     & 0.192             \\
\hline
7    & Light conditions   & 0.164          \\
\hline
8    & Pedestrian movement     & 0.148         \\
\hline
9    & Road surface type    & 0.136            \\
\hline

\end{tabular}
\caption{Feature importance ranking based on change frequency}
\label{tab:feature_importance}
\end{table}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{gl.png}
    \caption{Global Feature Change Frequency in Counterfactual Generation from 2000 Factual Instances.}
    \label{fig:gl}
\end{figure}

In the process of generating counterfactual instances, a higher change frequency demonstrates the importance of the corresponding feature in producing counterfactuals. The highest change frequencies for $Cause\ of\ accident$ and $Driving\ experience$ indicate that these two features are adjusted most often to flip a “severe” prediction. Moderate modification frequencies for $Type\ of\ collision$ and $Vehicle\ movement$ further highlight their influence on the model’s decisions. Intermediate change frequencies for $Weather\ conditions$, $Types\ of\ Junction$ and $Light\ conditions$ (0.164) show a secondary level of importance, while the lower frequencies for $Pedestrian\ movement$ and $Road\ surface\ type$ imply these features play a smaller role in counterfactual generation. Overall, this distribution of change frequencies reflects the degree to which the model relies on each feature when seeking minimal adjustments to alter its prediction. 


\subsection{Local and Region Feature Change Frequency}
A single factual instance was randomly selected, and its five nearest neighbors were identified to form a region consisting of six factual instances. For each instance, $10$ counterfactuals were generated. 

In the local feature frequency, the average change frequency and standard deviation for each feature were computed separately for six regions, shows in figures \ref{fig:overall}.


In Region $1$ figure \ref{fig:local1}, the average change frequency of $Driving\ experience$ is 0.23 (Std = 0.18), $Types\ of\ Junction$ is $0.43$ (Std = $0.21$), and $Type\ of\ collision$ is $0.43$ (Std = $0.29$). $Road\ surface \ type$ remains $0$ throughout this region, indicating that this feature was not modified at all. This pattern suggests that the counterfactual modifications in Region 1 predominantly focus on adjusting the features related to junction types and collision types, which are modified most frequently, while the driving experience is changed less often, and the road surface type plays no role in altering the prediction.


In Region $2$ figure \ref{fig:local2}, the value for $Type\ of\ collision$ is $0.53$; in Region $3$ figure \ref{fig:local3}, $Types\ of\ Junction$ and $Light\ conditions$ have values of $0.47$ and $0.2$7 respectively, while $Pedestrian\ movement$ is only $0.03$; in Region $4$ figure \ref{fig:local4}, both $Types\ of\ Junction$ and $Light\ conditions$ are likewise $0.47$ and $0.27$ respectively, and $Vehicle\ movement$ is $0.30$.

In Region $5$ figure \ref{fig:local5}, the average change frequency for $Types\ of\ Junction$ is significantly high at 0.56 (Std = 0.21), while the change in $Light\ Conditions$ is very small, at only 0.05 (Std = 0.03). In Region 6 figure \ref{fig:local6}, $Driving\ Experience$ remains high, with an average change frequency of 0.44 (Std = 0.17); however, $Types\ of\ Junction$ significantly drops to 0.25 (Std = 0.17), and $Road\ Surface\ Type$ remains extremely low at only 0.04 (Std = 0.02). The modification frequency for $Type\ of\ Collision$ increases to 0.42 (Std = 0.26), indicating a more significant impact on decision changes.



\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{chapters/chapter04/local1.png}
    \caption{Region 1}
    \label{fig:local1}
  \end{subfigure}%
  \hspace{0.5cm}
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{chapters/chapter04/local2.png}
    \caption{Region 2}
    \label{fig:local2}
  \end{subfigure}

  \vspace{0.7cm}
  
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{chapters/chapter04/local3.png}
    \caption{Region 3}
    \label{fig:local3}
  \end{subfigure}%
  \hspace{0.5cm}
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{chapters/chapter04/local4.png}
    \caption{Region 4}
    \label{fig:local4}
  \end{subfigure}
  \vspace{0.7cm}
  
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{chapters/chapter04/local5.png}
    \caption{Region 5}
    \label{fig:local5}
  \end{subfigure}%
  \hspace{0.5cm}
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.20\textheight]{chapters/chapter04/local6.png}
    \caption{Region 6}
    \label{fig:local6}
  \end{subfigure}
  
\caption{Average and standard deviation of local feature change frequencies computed for six regions, each formed by a randomly selected factual instance and its five nearest neighbors with $10$ counterfactuals generated per instance.}
\label{fig:overall}
\end{figure}









In Region $1$ and $2$, counterfactual explanations mainly rely on adjusting $Types\ of\ 
Junction$ and $Type\ of\ collision$, while $Road\ surface\ type$ remains unchanged in both regions, indicating that no modifications are made to pavement-related factors. In Region $2$, compared to Region $1$, the change frequency for $Type\ of\ collision$ is significantly higher, demonstrating a greater emphasis on adjustments related to collision type in that region. Both Region $3$ and Region $4$ exhibit a strong tendency to adjust $Types\ of\ Junction$ and $Light\ conditions$; however, in Region $3$, $Weather\ conditions$ are not modified at all and changes in $Pedestrian\ movement$ are minimal, whereas Region $4$ further incorporates adjustments to $Vehicle\ movement$ and $Cause\ of\ accident$, indicating some differences in local feature modifications between the two regions. 


Region $5$ displays a distinctly different pattern from the aforementioned regions, with counterfactual explanations tending to adjust $Road\ surface\ type$ and $Weather\ conditions$, which are directly related to the road and environmental factors, and a relatively lower reliance on $Driving\ experience$ and $Type\ of\ collision$. In Region $6$, the counterfactual modifications are primarily focused on $Driving\ experience$ and $Types\ of\ junction$, while the other features, especially $Cause\ of\ accident$, remain nearly stable, indicating that the changes in this region are mainly driven by driving behavior and junction types. 


These differences reflect significant variations in the emphasis the model places on different features when generating counterfactual explanations across these six regions, stemming from the varying feature distributions or characteristics of the sample groups in each region.

\section{Correlation Between Region and Global Frequency}
As shown in the figure \ref{fig:overallre}, the horizontal axis represents the Global Frequency, and the vertical axis represents the Local Frequency. By comparing the frequency values of each feature at the global and local levels within each region, the Pearson correlation coefficient ($r$ value) for each region is computed.

\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.25\textheight]{chapters/chapter04/re1.png}
    \caption{Correlation between region 1 and global feature change frequency}
    \label{fig:re1}
  \end{subfigure}%
  \hspace{0.5cm}
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.25\textheight]{chapters/chapter04/re2.png}
    \caption{Correlation between region 2 and global feature change frequency}
    \label{fig:re2}
  \end{subfigure}

  \vspace{0.1cm}
  
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.25\textheight]{chapters/chapter04/re3.png}
    \caption{Correlation between region 3 and global feature change frequency}
    \label{fig:re3}
  \end{subfigure}%
  \hspace{0.5cm}
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.25\textheight]{chapters/chapter04/re4.png}
    \caption{Correlation between region 4 and global feature change frequency}
    \label{fig:re4}
  \end{subfigure}
  \vspace{0.1cm}
  
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.25\textheight]{chapters/chapter04/re5.png}
    \caption{Correlation between region 5 and global feature change frequency}
    \label{fig:re5}
  \end{subfigure}%
  \hspace{0.5cm}
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[height=0.25\textheight]{chapters/chapter04/re6.png}
    \caption{Correlation between region 6 and global feature change frequency}
    \label{fig:re6}
  \end{subfigure}
  
\caption{The Pearson correlation coefficient between the feature change frequencies in the six regions and the Global data.}
\label{fig:overallre}
\end{figure}




From figure \ref{fig:re1}, for Region 1, the correlation coefficient with the global data is $r$ = 0.31. In the global dataset, the change frequencies of $Driving\ experience$ and $Cause\ of\ accident$ are relatively high, whereas in the local data these two exhibit relatively lower change frequencies, showing a ``high in global, low in local" pattern. In contrast, although the change frequencies of $Types\ of\ Junction$ and $Type\ of\ collision$ are not particularly prominent in the global data, they increase significantly in the local data, displaying a ``high in local, low in global" trend; meanwhile, $Road\ surface\ type$, $Light\ conditions$, $Weather\ conditions$, and $Pedestrian\ movement$ remain low in both the global and local datasets. This inconsistency in the ordering of change frequencies for some features results in only moderate overall agreement for Region 1, leading to an $r$ value of 0.31.

As shown in figure \ref{fig:re2}, for Region 2, the correlation coefficient with the global data is $r$ = 0.25. The change frequencies of $Driving\ experience$ and $Cause\ of\ accident$ are high in the global data, but they decrease in the local data, exhibiting a ``high globally, low locally" pattern. Meanwhile, the change frequencies of $Types\ of\ Junction$ and $Type\ of\ collision$ are significantly higher locally, displaying a ``high locally, low globally" trend. $Road\ surface\ type$, $Light\ conditions$, and $Weather\ conditions$ remain at low levels in both the global and local data. Since the ranking of change frequencies for some features does not fully correspond between the local and global data, the overall consistency of the ranking in Region 2 is weak, with an $r$ value of only 0.25.

As shown in the figure \ref{fig:re3}. In Region 3, the Pearson correlation coefficient between the local and global change frequencies is $r$ = 0.40. The variation frequency of $Types\ of\ Junction$ in the local region is significantly higher than in the global data, exhibiting a ``local high, global low" pattern, whereas $Driving\ experience$, which has a high variation frequency globally, is reduced locally, demonstrating a ``global high, local low" trend. In addition, both $Road\ surface\ type$ and $Weather\ conditions$ maintain low variation frequencies in both global and local data. Overall, the ranking of feature variation frequencies in Region 3 aligns well with the global baseline, which explains its relatively high $r$ value of 0.40.

As shown in the figure \ref{fig:re4}. In Region 4, the Pearson correlation coefficient between the local and global change frequencies is $r$ = 0.36, and the situation is similar to that in Region 3. $Driving\ experience$ originally exhibits a high change frequency at the global level, but its frequency decreases in the local data, forming a ``global high, local low" pattern. In contrast, $Types\ of\ Junction$ and $Light\ conditions$ increase from relatively low levels globally to much higher levels locally, displaying a ``local high, global low" pattern. $Road\ surface\ type$ and $Weather\ conditions$ remain low in both global and local settings, and $Type\ of\ collision$ is essentially unchanged between the two. This shift in the ordering of change frequencies for some features results in an overall moderate consistency in Region 4, with an $r$ value of 0.36.

As shown in the figure \ref{fig:re5}, The Pearson correlation coefficient between the local and global change frequencies of Region 5 is $r$ = -0.21, indicating a completely different distribution. In this region, the change frequency of $Driving\ experience$, which is high globally, is significantly reduced in the local data, exhibiting a ``globally high, locally low" pattern. In contrast, $Types\ of\ Junction$, $Road\ surface\ type$, $Weather\ conditions$, $Vehicle\ movement$, and $Pedestrian\ movement$, which have relatively low change frequencies in the global data, increase in the local data, showing a ``locally high, globally low" pattern. This complete reversal in overall ranking results in the ordering of feature change frequencies in Region 5 being almost entirely opposite to the global benchmark, leading to a negative $r$ value of -0.21.

Finally, as shown in the figure \ref{fig:re6}, Region 6 has a correlation of $r$ = 0.2$2$ with the global data. In this region, the change frequency for $Types\ of\ Junctio$n clearly increases locally, exhibiting a ``locally high, globally low" trend; whereas the change frequency for $Cause\ of\ acciden$t drops from a high global level to a lower local level, representing a ``globally high, locally low" pattern. In addition, $Light\ conditions$, $Weather\ conditions$, $Vehicle\ movement$, and $Pedestrian\ movement$ are relatively low in both global and local contexts. Due to the significant changes in some key features in the local data, the overall consistency of Region 6 is weakened, resulting in an $r$ value of only 0.2$2$.
\section{Modification Sparsity}
In the global feature modification sparsity analysis, the figure \ref{fig:xishu} shows the distribution of the number of modified features across all counterfactual instances: the counterfactual with two modified features is the most frequent, with $1216$ instances; 338 instances have three modified features, while $230$ instances have only one modified feature; the numbers of instances for four, five, six, and seven modified features are $104$, $60$, $30$, and $22$, respectively. This indicates that in most counterfactual instances, only a relatively small number of features are modified, primarily concentrated in the range of one to three features.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{xishu.png}
    \caption{ Distribution of the number of modified features in counterfactual instances generated from $2000$ factual cases, with modifications ranging from one to seven features.}
    \label{fig:xishu}
\end{figure}


This model exhibits good sparsity as most counterfactual instances require only modifying one to three features to change the prediction from ``severe" to ``non-severe". This not only makes the explanation more intuitive but also aligns with real-world scenarios, where users or decision-makers typically can only adjust a limited number of controllable factors. Sparse and clear explanations can better guide practical interventions, thereby enhancing the operability of accident prevention measures.

\section{Mode}
The original factual samples from Region $1$ are compared with their generated counterfactual samples, focusing on the proportion of the mode for each feature.
\begin{table}[htbp]
\centering

\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|r|}
\hline
\textbf{Feature} & \textbf{Original Mode} & \textbf{Mode \%} & \textbf{Original Mode \% in CF  } &\delta_j \\
\hline

Driving experience      & Below 1yr                    & 66.67\%   & 55.00\%      &-0.175\\
\hline
Types of Junction      & Crossing                     & 83.33\%   & 60.00\%   &-0.28 \\
\hline
Road surface type       & Asphalt roads                & 100.00\%  & 100.00\%   &0\\
\hline
Light conditions        & Darkness - lights lit        & 100.00\%  & 85.00\%   &-0.15 \\
\hline
Weather conditions      & Normal                       & 100.00\%  & 98.33\%    &-0.017 \\
\hline
Type of collision      & Vehicle with vehicle collision & 100.00\% & 45.00\%  &-0.55\\
\hline
Vehicle movement        & Going straight               & 100.00\%  & 68.33\%   &-0.317\\
\hline
Pedestrian movement     & Not a Pedestrian             & 50.00\%   & 46.67\%     &-0.067 \\
\hline
Cause of accident      & No priority to pedestrian    & 50.00\%   & 41.67\%   &-0.167 \\
\hline

\end{tabular}%
}
\caption{Comparison of Mode Categories and Percentages in Original and Counterfactual Samples of Region $1$. Original Mode: Refers to the most frequent category for each feature in the original instances. Mode $\%$: Represents the percentage of the Original Mode. Original Mode $\%$ in CF: Indicates the percentage of the Original Mode in the counterfactual instances. $\delta_j$: Relative change rate from equation}
\label{tab:mode_comparison}
\end{table}



The table \ref{tab:mode_comparison} shows that the mode for each feature in the original data still holds the highest proportion in the counterfactual samples, although the overall percentages show a slight decline, meaning that all $\delta_j$ is negative or zero.

Among them, $Type\ of\ collision$ has a $\delta_j$ of $–0.55$, with an absolute value much higher than that of the other features. This indicates that during the counterfactual generation process, the proportion of the dominant category “Vehicle with vehicle collision” for $Type\ of\ collision$ experienced a significant change, suggesting that it may be the main factor driving the prediction from “severe” to “non-severe”, that make $Type\ of\ collision$ has high change frequency in Region $1$. 

Another feature in Region $1$ with a high change frequency is $Types\ of\ Junction$, whose $|\delta_j|$ is 0.28, which is still relatively high, but only half that of $Type\ of\ collision$. This demonstrates that the dominant category ‘Crossing’ for $Types\ of\ Junction$ is a relatively less important factor in causing the prediction to switch from “severe” to “non-severe”. 

In contrast, $Weather\ conditions$ and $Road\ surface\ type$ have $|\delta_j|$ values of $0.017$ and $0.00$, respectively, indicating that the dominant categories for these two features have little to no impact on the prediction change, which is why these two features have the lowest change frequencies.

==> chapters/chapter05/chap05.tex <==
\chapter{Limitations and Future Work}
\section{Limitations}
\subsection{Dataset}
The accident record data used in this study were only collected from Addis Ababa Sub-city, and the data collection period is limited to 2017–2020. This geographical limitation means that the traffic accident cases included in the dataset only reflect the specific regional characteristics such as local traffic conditions, driving habits, road infrastructure, climate, and related safety management measures, which may differ significantly from those in other regions. For example, road design, traffic volume, enforcement intensity, and public transportation facilities in other cities or rural areas may vary considerably, potentially affecting the accident prediction and explanation performance of the same model when applied elsewhere. In addition, the limited time span of the data may prevent the study from capturing long-term trends or cyclical fluctuations in traffic accident patterns over time, thereby impacting the model's generalizability to scenarios beyond the historical data. In summary, these geographical and temporal limitations may result in the model performing less consistently in a broader range of application contexts, thereby affecting its generalizability and reliability.
\subsection{Uncertainty in Counterfactual Generation}
The study primarily relies on the DiCE algorithm to generate counterfactual explanations. Although the algorithm performs exceptionally well in maintaining the sparsity and feasibility of counterfactual explanations, allowing the model's prediction to be changed through relatively few feature modifications, the generated results may in some cases fail to truly capture the causal relationships between variables. In other words, while adjusting certain input features can change the model’s prediction, such changes may not necessarily reflect the actual causal mechanisms, and may therefore differ from the true causal effects.

Moreover, the stability of the generated counterfactual results faces significant challenges. Since the generation process is highly dependent on the initial state of the input data and the model parameters, its outcomes can be affected by several factors. First, the influence of input perturbations on the results is not negligible, as even minor data noise or slight perturbations may lead to substantial changes in the generated counterfactual instances, thereby reducing the robustness of the explanations. Second, as the model undergoes updates or retraining, changes in the internal decision boundaries may render previously generated counterfactual explanations ineffective, which can compromise the consistency of the interpretations. Finally, the algorithm's hyperparameters are highly sensitive in the counterfactual generation process; different settings may result in significant variations in minimizing feature modifications or ensuring the diversity of the generated counterfactuals, ultimately causing the final explanation results to exhibit instability across repeated experiments.
\subsection{Inability to Effectively Normalize Nominal Categorical Data}
The majority of data used in this study are nominal data, which refers to data in which the categories have no inherent order or metric, such as $Types\ of\ Junctio$ and $Vehicle\ movement$. These categories are only used to represent different types or states and do not contain any quantitative or ordinal information. Traditional normalization methods, such as min-max scaling or standardization, are primarily designed for continuous numerical attributes or data with an inherent order, and therefore cannot be directly applied to nominal data. Although label encoding can be used to convert these categories into numerical values, this approach implicitly introduces an artificial order that does not reflect the actual similarities or differences among the categories. As a result, during the distance-based counterfactual generation process, such an unjustified order can lead to biases in the distance calculations, causing certain categories to be mistakenly evaluated as more dissimilar than they truly are. This bias ultimately impacts the accuracy of feature modification judgments and the objectivity of the explanation process, thereby undermining the effectiveness and reliability of the counterfactual explanation method.


\section{Future Work}
\subsection{Data expansion and diversity enhancement}
Future research could consider collecting traffic accident data from a broader range of geographical areas, including different cities, countries, and even regions with varied climate zones, in order to capture a more diverse range of road structures, traffic flows, driving behaviors, and environmental factors. Additionally, the data collection period should be extended in the time dimension to include not only recent accident data but also historical data, thereby more comprehensively reflecting the long-term trends and changes in traffic accidents. In terms of data diversity, relying solely on text or numerical data may not be sufficient to reveal all the complex factors underlying traffic accidents. Thus, future work should actively incorporate multi-modal data, such as traffic surveillance videos, vehicle sensor data, GPS trajectories, and other real-time data related to the traffic environment, to understand the dynamic processes and potential causal relationships behind accidents from multiple perspectives, thereby improving the accuracy and practical applicability of counterfactual explanations. By combining the visual information from video images with the real-time dynamics of sensor data, the model can obtain a more comprehensive representation during training, thereby enhancing its robustness and generalization capabilities.
\subsection{Evaluation Metrics – Necessity and Sufficiency}
One promising direction is to incorporate and investigate additional evaluation metrics for counterfactual explanations, particularly focusing on sufficiency and necessity. Inspired by the framework proposed in \cite{kommiya2021towards}, future work will quantitatively assess whether the key features identified are both necessary for, and sufficient to maintain, the original predictions. By adapting metrics that capture the conditional probability of feature relevance (sufficiency) and the impact of feature modification (necessity), we aim to provide a more robust sensitivity analysis of the explanations. This sensitivity study would evaluate how small perturbations in the input or model parameters affect the counterfactual outcomes.

\subsection{ Exploring Alternative Counterfactual Generation Methods and Machine Learning Models}
While the current work utilizes DiCE with a Random Forest model, it would be beneficial to compare the performance and stability of different counterfactual generation approaches. Future studies will evaluate alternative methods such as WachterCF and newer algorithms that may integrate causal inference or graph based techniques. In addition, applying different machine learning models, ranging from simpler logistic regression and multilayer perceptrons (MLP) to other ensemble methods, will help determine the generalizability and robustness of the counterfactual explanations under various modeling paradigms. This exploration is expected to shed light on the sensitivity of the explanation quality when the underlying model architecture changes.

==> chapters/chapter06/chap06.tex <==
\chapter{Conclusion}
A global and local counterfactual explanation framework has been developed for a random forest classifier trained on 12316 samples with 12 features drawn from manual records of road traffic accidents in the Addis Ababa Sub‑city police departments during the years 2017 to 2020. The classifier achieved an F1 score of 0.789 and an overall accuracy of 83.5$\%$, demonstrating strong performance on imbalanced severity data.

Global analysis showed that the features $Cause\ of\ accident$, and $Driving\ experience$ require the most frequent adjustments to change a prediction from ``severe" to ``non severe", yielding a clear ranking of overall importance. Local analysis, by generating multiple counterfactuals for each case and its nearest neighbors, revealed case‑specific severity drivers and produced Pearson correlation values between global and local rankings ranging from –0.21 to 0.40, indicating that individual contexts can differ markedly from aggregate trends. Sparsity assessment confirmed that most explanations modify only one to three features, and mode‑shift analysis identified collision type as the feature with the largest change in dominant category.

These findings show that counterfactual explanations can clarify the decision logic of a black box accident severity model and offer concise, actionable guidance, such as targeted speed reductions and improvements to road conditions, to help mitigate severe outcomes. By quantifying both overall feature importance and local variability, this approach supports policy making and driver advisories that are tailored to specific risk profiles.

Future work should enlarge the geographic and temporal scope of the dataset, strengthen the causal validity and stability of generated counterfactuals, and investigate normalization strategies for nominal features. Integrating multi modal traffic data, applying necessity and sufficiency metrics, and exploring alternative generation methods promise to further enhance the reliability and utility of counterfactual explanations in traffic safety applications.








==> frontmatter/abstract.tex <==
%
% File: abstract.tex
% Author: V?ctor Bre?a-Medina
% Description: Contains the text for thesis abstract
%
% UoB guidelines:
%
% Each copy must include an abstract or summary of the dissertation in not
% more than 300 words, on one side of A4, which should be single-spaced in a
% font size in the range 10 to 12. If the dissertation is in a language other
% than English, an abstract in that language and an abstract in English must
% be included.

\chapter*{Abstract}
\begin{SingleSpace}
This study develops a global and local counterfactual explanation framework for a random forest classifier trained on 12316 manually recorded traffic accident cases with 12 categorical features from the Addis Ababa Sub city police departments, an administrative subdivision of Addis Ababa, the capital city of Ethiopia in East Africa, over the years 2017 to 2020. The classifier achieved an F1 score of 0.789 and an accuracy of 83.5$\%$ in distinguishing severe from non severe collisions. Counterfactual instances were generated using the DiCE library to simulate minimal feature adjustments required to change a prediction from “severe” to “non severe.” In global analysis, features were ranked by the frequency of required modifications, with driving experience, collision type and cause of accident identified as most influential. In local analysis, multiple counterfactuals were generated for each case and its five nearest neighbors to identify and quantify the key factors specific to each case that most influence accident severity, with Pearson correlation coefficients between global feature importance rankings and local feature importance rankings across six regions ranging from –0.21 to 0.40. Sparsity assessment showed that 70 percent of explanations alter only one to three features, and mode shift analysis highlighted collision type as having the largest change in dominant category. These results demonstrate that counterfactual explanations can both illuminate the internal logic of a black box accident severity model and provide concise actionable insights, such as targeted speed reductions and improvements to road conditions, to mitigate severe outcomes. Future work should focus on expanding the geographic scope to access the generalisability of the presented finding, enhancing causal validity and integrating multi modal data to further strengthen interpretability in traffic safety applications.
\end{SingleSpace}
\clearpage

==> frontmatter/declaration.tex <==
%
% File: declaration.tex
% Author: V?ctor Bre?a-Medina
% Description: Contains the declaration page
%
% UoB guidelines:
%
% Author's declaration
%
% I declare that the work in this dissertation was carried out in accordance
% with the requirements of the University's Regulations and Code of Practice
% for Research Degree Programmes and that it has not been submitted for any
% other academic award. Except where indicated by specific reference in the
% text, the work is the candidate's own work. Work done in collaboration with,
% or with the assistance of, others, is indicated as such. Any views expressed
% in the dissertation are those of the author.
%
% SIGNED: .............................................................
% DATE:..........................
%
\chapter*{Ethics and AI declaration}
\begin{SingleSpace}
\begin{quote}
The Project is covered under blanket ethics.

\vspace{1.5cm}


In this report, AI was used helping to make writing more concise and professional.
\noindent

\end{quote}
\end{SingleSpace}
\clearpage

==> frontmatter/dedication.tex <==
%
% file: dedication.tex
% author: V?ctor Bre?a-Medina
% description: Contains the text for thesis dedication
%

\chapter*{Dedication and acknowledgements}
\begin{SingleSpace}
Here goes the dedication.
\end{SingleSpace}
\clearpage

==> frontmatter/title.tex <==
%
% File: Title.tex
% Author: V?ctor Bre?a-Medina
% Description: Contains the title page
%
% UoB guidelines:
% 
% At the top of the title page, within the margins, the dissertation should give the title and, if 
% necessary, sub-title and volume number. If the dissertation is in a language other than English, the 
% title must be given in that language and in English. The full name of the author should be in the 
% centre of the page. At the bottom centre should be the words ?A dissertation submitted to the 
% University of Bristol in accordance with the requirements for award of the degree of ? in the 
% Faculty of ...?, with the name of the school and month and year of submission. The word count of 
% the dissertation (text only) should be entered at the bottom right-hand side of the page.
%
%
\begin{titlingpage}
\begin{SingleSpace}
\calccentering{\unitlength} 
\begin{adjustwidth*}{\unitlength}{-\unitlength}
\vspace*{13mm}
\begin{center}
\rule[0.5ex]{\linewidth}{2pt}\vspace*{-\baselineskip}\vspace*{3.2pt}
\rule[0.5ex]{\linewidth}{1pt}\\[\baselineskip]
{\HUGE Predicting Reduced Accident Severity Via Counterfactual Explanations }\\[4mm]
{\Large \textit{A Global And Local Feature Analysis Approach}}\\
\rule[0.5ex]{\linewidth}{1pt}\vspace*{-\baselineskip}\vspace{3.2pt}
\rule[0.5ex]{\linewidth}{2pt}\\
\vspace{6.5mm}
{\large By}\\
\vspace{6.5mm}
{\large\textsc{Yixuan Zhou}}\\
\vspace{11mm}
\includegraphics[scale=0.6]{logos/bristolcrest_colour}\\
\vspace{6mm}
{\large Department of Engineering Mathematics\\
\textsc{University of Bristol}}\\
\vspace{11mm}
\begin{minipage}{10cm}
Project Report submitted in support of the degree of Master of Engineering
\end{minipage}\\
\vspace{9mm}
{\large\textsc{April 2025}}
\vspace{12mm}
\end{center}

\end{adjustwidth*}
\end{SingleSpace}
\end{titlingpage}
